Tamagawa Products for Elliptic Curves Over Number Fields

In recent work, Griffin, Ono, and Tsai constructs an $L-$series to prove that the proportion of short Weierstrass elliptic curves over $\mathbb{Q}$ with trivial Tamagawa product is $0.5054\dots$ and that the average Tamagawa product is $1.8183\dots$. Following their work, we generalize their $L-$series over arbitrary number fields $K$ to be \[L_{\mathrm{Tam}}(K; s):=\sum_{m=1}^{\infty}\frac{P_{\mathrm{Tam}}(K; m)}{m^s},\] where $P_{\mathrm{Tam}}(K;m)$ is the proportion of short Weierstrass elliptic curves over $K$ with Tamagawa product $m$. We then construct Markov chains to compute the exact values of $P_{\mathrm{Tam}}(K;m)$ for all number fields $K$ and positive integers $m$. As a corollary, we also compute the average Tamagawa product $L_{\mathrm{Tam}}(K;-1)$. We then use these results to uniformly bound $P_{\mathrm{Tam}}(K;1)$ and $L_{\mathrm{Tam}}(K,-1)$ in terms of the degree of $K$. Finally, we show that there exist sequences of $K$ for which $P_{\mathrm{Tam}}(K;1)$ tends to $0$ and $L_{\mathrm{Tam}}(K;-1)$ to $\infty$, as well as sequences of $K$ for which $P_{\mathrm{Tam}}(K;1)$ and $L_{\mathrm{Tam}}(K;-1)$ tend to $1$.

==> data.tex <==
Real Quardratic Fields Trivial Tamagawa Numbers, D < 10000

55, 51, 71, 48, 46, 45, 51, 62, 51, 48, 35, 44, 63, 45, 53, 52, 67, 48, 43, 32, 43, 53, 59, 55, 46, 33, 50, 45, 42, 56, 46, 70, 44, 31, 45, 52, 57, 56, 33, 47, 45, 62, 44, 50, 29, 50, 72, 49, 42, 46, 57, 58, 50, 51, 33, 42, 65, 43, 52, 29, 68, 49, 46, 31, 42, 54, 56, 54, 47, 33, 46, 45, 46, 51, 56, 50, 45, 30, 43, 52, 60, 50, 34, 52, 43, 61, 45, 57, 28, 52, 67, 42, 43, 52, 60, 54, 47, 32, 45, 63, 43, 57, 52, 74, 48, 31, 46, 50, 57, 56, 50, 33, 46, 46, 43, 49, 28, 52, 50, 72, 43, 30, 46, 55, 57, 53, 32, 48, 42, 67, 42, 55, 29, 53, 46, 66, 52, 46, 42, 57, 57, 54, 47, 34, 43, 68, 46, 51, 27, 45, 44, 29, 51, 59, 50, 50, 34, 51, 42, 46, 54, 28, 52, 49, 68, 43, 31, 42, 59, 56, 32, 50, 47, 65, 43, 54, 53, 46, 75, 43, 44, 53, 56, 53, 50, 33, 47, 60, 44, 51, 29, 53, 71, 52, 42, 30, 45, 54, 50, 52, 32, 48, 42, 43, 54, 28, 47, 68, 30, 43, 54, 57, 35, 46, 44, 66, 45, 51, 57, 69, 46, 46, 45, 52, 59, 52, 35, 42, 63, 45, 56, 28, 49, 65, 49, 43, 31, 41, 55, 61, 58, 46, 31, 52, 45, 42, 54, 27, 52, 48, 73, 43, 31, 47, 52, 55, 54, 48, 45, 60, 44, 51, 29, 51, 48, 75, 49, 43, 45, 53, 57, 52, 53, 31, 43, 69, 43, 53, 28, 57, 69, 51, 44, 30, 42, 55, 56, 53, 46, 34, 48, 44, 53, 27, 56, 51, 68, 45, 30, 50, 61, 50, 34, 49, 42, 61, 47, 57, 27, 50, 68, 49, 42, 43, 52, 61, 55, 46, 32, 47, 42, 55, 54, 71, 46, 45, 32, 47, 56, 55, 49, 34, 47, 45, 52, 28, 50, 47, 72, 43, 29, 44, 57, 59, 52, 31, 49, 42, 67, 43, 29, 48, 67, 50, 45, 43, 56, 55, 53, 48, 35, 43, 64, 46, 49, 27, 56, 46, 47, 29, 43, 51, 59, 51, 50, 34, 51, 43, 47, 56, 53, 49, 70, 41, 32, 42, 56, 53, 31, 51, 47, 63, 42, 55, 27, 47, 70, 47, 44, 46, 50, 57, 54, 51, 33, 45, 60, 45, 52, 28, 50, 75, 52, 42, 29, 47, 54, 58, 50, 33, 48, 43, 42, 53, 28, 55, 48, 66, 47, 30, 43, 55, 55, 55, 35, 47, 43, 69, 44, 51, 27, 50, 46, 43, 51, 62, 53, 34, 42, 63, 45, 55, 28, 50, 67, 41, 31, 44, 55, 58, 54, 48, 33, 52, 45, 43, 54, 27, 53, 45, 74, 31, 45, 50, 55, 56, 32, 46, 47, 63, 44, 52, 28, 53, 47, 73, 51, 42, 45, 56, 58, 50, 48, 31, 44, 66, 42, 53, 29, 55, 67, 52, 44, 42, 55, 56, 52, 48, 46, 43, 48, 52, 54, 53, 29, 50, 62, 51, 35, 50, 42, 61, 44, 54, 27, 53, 66, 47, 43, 43, 60, 56, 47, 32, 44, 64, 42, 57, 27, 53, 71, 47, 45, 31, 45, 53, 57, 56, 50, 32, 47, 44, 44, 50, 29, 50, 51, 72, 42, 29, 46, 57, 50, 32, 51, 64, 44, 52, 29, 55, 45, 70, 50, 47, 42, 54, 55, 47, 34, 45, 68, 46, 51, 56, 72, 46, 45, 30, 43, 52, 60, 50, 34, 51, 43, 45, 57, 28, 53, 51, 66, 41, 32, 42, 52, 61, 55, 32, 49, 46, 62, 43, 57, 26, 52, 48, 73, 44, 46, 51, 57, 56, 49, 46, 43, 50, 28, 53, 70, 49, 43, 30, 47, 54, 57, 52, 51, 32, 42, 41, 55, 28, 46, 66, 47, 29, 42, 56, 57, 53, 34, 49, 69, 50, 27, 53, 71, 47, 44, 44, 53, 58, 50, 50, 35, 43, 60, 47, 54, 28, 51, 68, 49, 43, 32, 41, 52, 59, 56, 48, 31, 49, 46, 43, 26, 54, 46, 75, 43, 32, 44, 53, 56, 55, 32, 49, 46, 61, 53, 29, 52, 49, 72, 51, 42, 47, 55, 60, 50, 51, 32, 41, 66, 43, 28, 54, 69, 50, 30, 43, 54, 57, 54, 46, 35, 46, 45, 45, 50, 26, 56, 51, 69, 47, 30, 51, 58, 52, 35, 51, 41, 63, 44, 56, 50, 50, 68, 50, 43, 42, 54, 61, 57, 47, 31, 45, 65, 42, 54, 27, 74, 46, 43, 30, 46, 52, 55, 54, 52, 34, 48, 46, 44, 50, 29, 73, 43, 29, 45, 54, 57, 53, 32, 47, 43, 69, 44, 55, 28, 57, 45, 67, 51, 44, 42, 56, 56, 51, 46, 33, 46, 65, 44, 53, 27, 56, 48, 45, 29, 44, 62, 50, 48, 35, 50, 42, 46, 55, 27, 50, 51, 69, 42, 31, 43, 53, 61, 54, 32, 49, 47, 64, 42, 54, 55, 49, 70, 46, 46, 50, 55, 57, 50, 34, 44, 63, 43, 52, 29, 50, 72, 51, 44, 28, 45, 56, 59, 52, 50, 31, 50, 41, 43, 52, 29, 55, 48, 45, 43, 56, 55, 52, 35, 47, 44, 66, 48, 50, 27, 54, 50, 45, 47, 51, 58, 53, 49, 33, 44, 62, 47, 55, 27, 51, 70, 42, 32, 42, 60, 53, 45, 31, 52, 46, 41, 57, 27, 54, 47, 72, 43, 32, 45, 50, 57, 55, 33, 47, 44, 61, 45, 51, 28, 51, 50, 74, 51, 46, 55, 51, 49, 32, 43, 66, 41, 53, 28, 55, 66, 50, 46, 31, 43, 56, 55, 46, 36, 47, 43, 46, 52, 27, 54, 49, 68, 46, 29, 43, 53, 52, 33, 52, 42, 64, 45, 54, 28, 51, 66, 48, 42, 44, 54, 60, 54, 47, 33, 46, 64, 44, 54, 27, 54, 74, 47, 44, 45, 50, 54, 55, 52, 45, 48, 45, 51, 28, 52, 48, 73, 41, 30, 44, 56, 58, 51, 32, 43, 65, 41, 54, 29, 56, 47, 66, 51, 45, 54, 58, 52, 49, 34, 65, 47, 53, 72, 47, 45, 29, 50, 62, 48, 35, 49, 43, 45, 54, 27, 52, 52, 66, 44, 32, 43, 58, 57, 32, 52, 46, 41, 56, 27, 51, 46, 71, 45, 44, 52, 56, 56, 50, 33, 45, 63, 50, 29, 50, 74, 49, 42, 29, 48, 57, 56, 51, 52, 32, 51, 42, 43, 29, 55, 47, 69, 46, 30, 41, 53, 55, 55, 33, 46, 45, 67, 46, 52, 26, 56, 49, 47, 45, 43, 52, 51, 34, 43, 60, 45, 56, 53, 65, 49, 42, 32, 42, 52, 61, 54, 49, 32, 49, 45, 43, 56, 48, 74, 44, 31, 47, 58, 34, 46, 47, 61, 44, 49, 28, 52, 73, 50, 43, 46, 56, 56, 51, 50, 32, 42, 68, 42, 53, 28, 54, 65, 52, 47, 30, 41, 55, 58, 55, 34, 48, 43, 46, 50, 27, 50, 45, 29, 45, 53, 59, 49, 35, 52, 42, 60, 47, 55, 28, 52, 49, 69, 43, 42, 53, 60, 56, 47, 31, 46, 67, 43, 54, 26, 54, 72, 47, 32, 45, 53, 55, 55, 50, 32, 48, 47, 43, 52, 29, 52, 49, 72, 42, 30, 45, 54, 58, 50, 48, 41, 66, 42, 55, 28, 54, 48, 70, 51, 44, 53, 57, 54, 46, 35, 45, 67, 44, 50, 26, 56, 69, 46, 47, 29, 51, 59, 53, 47, 42, 45, 56, 28, 50, 51, 66, 43, 31, 42, 61, 57, 31, 51, 44, 67, 43, 54, 27, 52, 48, 72, 45, 43, 48, 52, 55, 54, 52, 33, 61, 44, 51, 29, 52, 74, 49, 44, 29, 45, 54, 52, 51, 31, 49, 44, 43, 53, 28, 56, 46, 69, 45, 31, 41, 57, 56, 34, 47, 45, 64, 45, 52, 27, 57, 51, 69, 44, 43, 50, 62, 50, 35, 42, 60, 47, 56, 27, 51, 69, 50, 43, 30, 42, 53, 54, 47, 32, 50, 47, 42, 55, 54, 47, 72, 45, 32, 47, 51, 56, 57, 46, 44, 64, 44, 52, 28, 50, 48, 70, 52, 43, 45, 57, 58, 52, 50, 31, 42, 67, 53, 29, 53, 68, 50, 45, 30, 43, 56, 55, 52, 47, 36, 48, 46, 50, 27, 55, 50, 72, 46, 29, 44, 49, 59, 53, 33, 50, 64, 46, 27, 53, 51, 70, 48, 41, 41, 54, 61, 55, 46, 31, 47, 41, 56, 27, 54, 71, 49, 43, 32, 46, 51, 56, 55, 51, 33, 46, 45, 54, 28, 50, 49, 73, 42, 29, 46, 53, 59, 32, 47, 44, 68, 42, 28, 56, 47, 66, 49, 47, 44, 56, 55, 55, 45, 35, 43, 69, 45, 52, 54, 69, 48, 47, 29, 43, 53, 61, 51, 49, 34, 51, 42, 46, 54, 51, 51, 67, 42, 31, 43, 53, 60, 55, 33, 52, 45, 63, 43, 53, 27, 46, 74, 46, 46, 44, 51, 55, 56, 52, 32, 46, 62, 45, 52, 28, 52, 75, 50, 41, 30, 45, 57, 59, 50, 49, 31, 49, 43, 42, 53, 29, 56, 66, 45, 31, 42, 55, 57, 53, 34, 46, 43, 65, 47, 52, 26, 54, 48, 45, 49, 61, 50, 36, 43, 45, 55, 27, 52, 66, 43, 32, 44, 53, 58, 56, 47, 32, 50, 45, 41, 56, 27, 53, 46, 72, 30, 44, 52, 58, 56, 32, 47, 45, 63, 44, 50, 29, 50, 51, 51, 41, 47, 56, 57, 51, 52, 32, 42, 66, 43, 53, 29, 56, 69, 49, 46, 42, 53, 55, 54, 48, 33, 46, 45, 46, 51, 26, 57, 49, 45, 29, 52, 60, 50, 34, 52, 44, 60, 56, 28, 52, 50, 66, 50, 41, 42, 60, 54, 48, 32, 46, 63, 44, 56, 26, 52, 74, 48, 31, 47, 50, 57, 55, 49, 34, 46, 46, 43, 50, 28, 53, 49, 71, 44, 29, 46, 56, 51, 32, 49, 41, 67, 42, 55, 28, 46, 67, 51, 46, 42, 56, 58, 47, 33, 42, 69, 46, 50, 27, 53, 70, 45, 45, 29, 44, 53, 58, 51, 35, 51, 42, 47, 28, 50, 49, 70, 43, 41, 52, 59, 56, 32, 50, 47, 65, 43, 55, 54, 46, 75, 47, 44, 44, 52, 55, 54, 50, 47, 61, 43, 51, 29, 53, 71, 51, 42, 30, 54, 60, 51, 51, 32, 42, 43, 55, 28, 54, 48, 68, 45, 30, 44, 55, 56, 53, 45, 66, 45, 51, 26, 56, 68, 46, 46, 59, 52, 48, 35, 42, 64, 44, 56, 27, 51, 65, 51, 43, 30, 42, 54, 63, 56, 47, 31, 51, 45, 42, 54, 27, 52, 48, 73, 43, 30, 47, 52, 54, 53, 34, 48, 46, 60, 50, 29, 51, 48, 74, 51, 43, 44, 54, 57, 53, 52, 32, 43, 66, 43, 28, 57, 68, 51, 45, 31, 41, 57, 51, 46, 33, 47, 45, 46, 53, 27, 57, 50, 70, 44, 30, 45, 51, 61, 51, 34, 49, 41, 61, 47, 56, 49, 52, 69, 49, 43, 43, 53, 61, 45, 32, 47, 63, 42, 54, 26, 73, 46, 46, 32, 46, 50, 55, 56, 49, 34, 48, 44, 43, 53, 28, 50, 71, 44, 28, 45, 56, 58, 53, 31, 50, 42, 68, 42, 51, 29, 54, 49, 69, 49, 44, 43, 55, 55, 52, 47, 35, 45, 64, 47, 50, 27, 55, 47, 46, 29, 43, 51, 59, 53, 50, 34, 50, 43, 47, 56, 27, 49, 68, 42, 32, 42, 53, 61, 53, 31, 51, 46, 64, 41, 57, 27, 55, 46, 71, 46, 57, 53, 51, 45, 61, 45, 52, 28, 50, 74, 51, 42, 28, 46, 55, 59, 51, 50, 33, 47, 42, 51, 28, 57, 49, 65, 46, 43, 55, 55, 55, 35, 43, 68, 44, 52, 26, 55, 49, 69, 47, 46, 52, 62, 52, 49, 34, 41, 63, 46, 55, 28, 50, 68, 48, 42, 31, 44, 59, 55, 47, 32, 51, 44, 54, 27, 52, 47, 73, 46, 32, 44, 50, 54, 56, 32, 46, 47, 63, 46, 51, 28, 51, 47, 75, 51, 42, 45, 56, 50, 49, 31, 42, 66, 41, 55, 29, 56, 66, 51, 46, 30, 43, 54, 57, 47, 34, 47, 43, 46, 52, 26, 52, 73, 45, 29, 44, 50, 63, 52, 35, 50, 43, 45, 54, 27, 52, 52, 65, 48, 43, 43, 54, 58, 57, 46, 33, 45, 66, 42, 56, 26, 52, 71, 48, 44, 31, 45, 52, 57, 56, 51, 47, 46, 50, 29, 51, 49, 73, 42, 28, 47, 56, 57, 50, 33, 43, 66, 43, 51, 29, 55, 45, 70, 50, 47, 41, 54, 55, 54, 49, 34, 67, 47, 57, 70, 47, 44, 30, 43, 52, 60, 50, 49, 34, 51, 43, 44, 56, 28, 52, 50, 42, 32, 42, 53, 62, 54, 32, 49, 44, 43, 56, 26, 53, 48, 75, 48, 43, 47, 50, 58, 56, 49, 33, 47, 50, 28, 52, 71, 49, 43, 30, 46, 56, 57, 52, 50, 32, 49, 42, 42, 53, 45, 67, 47, 30, 42, 56, 56, 54, 34, 49, 43, 67, 45, 51, 27, 53, 52, 70, 46, 46, 52, 58, 51, 50, 34, 42, 61, 47, 53, 69, 43, 31, 41, 52, 59, 57, 47, 31, 49, 47, 43, 55, 26, 47, 73, 43, 31, 46, 52, 56, 55, 32, 48, 46, 61, 43, 53, 29, 52, 72, 51, 42, 46, 53, 60, 50, 52, 31, 41, 65, 43, 55, 28, 69, 52, 29, 43, 54, 57, 53, 46, 36, 46, 45, 49, 55, 52, 46, 30, 44, 52, 59, 52, 36, 50, 42, 62, 45, 56, 27, 51, 50, 66, 41, 54, 56, 47, 31, 45, 65, 42, 53, 27, 53, 45, 31, 46, 52, 56, 53, 52, 34, 48, 45, 45, 51, 29, 52, 47, 74, 43, 29, 46, 55, 57, 52, 31, 47, 43, 68, 44, 53, 28, 56, 46, 67, 45, 41, 57, 56, 53, 46, 34, 45, 66, 45, 52, 27, 56, 69, 49, 45, 30, 50, 61, 50, 49, 34, 49, 42, 46, 57, 27, 50, 52, 70, 30, 43, 60, 55, 32, 50, 46, 65, 41, 26, 55, 48, 72, 46, 44, 47, 51, 55, 57, 49, 34, 46, 62, 43, 52, 29, 49, 71, 52, 43, 29, 45, 56, 52, 51, 31, 49, 41, 43, 52, 29, 54, 47, 68, 44, 30, 44, 57, 54, 34, 48, 45, 66, 47, 51, 27, 55, 49, 71, 46, 48, 44, 60, 51, 34, 43, 64, 46, 56, 27, 52, 70, 49, 41, 41, 54, 60, 54, 46, 31, 52, 46, 42, 55, 27, 55, 47, 70, 43, 32, 51, 57, 55, 46, 44, 60, 45, 51, 28, 50, 50, 74, 51, 43, 46, 55, 60, 50, 32, 43, 66, 42, 52, 28, 57, 67, 50, 46, 31, 43, 56, 54, 46, 34, 47, 45, 51, 26, 53, 50, 68, 48, 29, 43, 52, 61, 52, 34, 51, 42, 63, 46, 55, 28, 50, 68, 48, 42, 54, 58, 53, 48, 33, 45, 43, 55, 27, 52, 74, 46, 45, 31, 45, 50, 55, 57, 51, 33, 46, 46, 50, 28, 53, 49, 75, 41, 29, 45, 55, 51, 31, 49, 44, 65, 41, 29, 56, 48, 66, 52, 44, 42, 54, 56, 52, 48, 35, 43, 66, 47, 53, 26, 54, 48, 46, 29, 45, 50, 61, 47, 35, 49, 44, 44, 55, 53, 51, 65, 44, 32, 43, 59, 56, 32, 51, 45, 67, 42, 56, 26, 46, 73, 48, 44, 45, 53, 56, 56, 32, 45, 63, 45, 50, 29, 51, 73, 50, 42, 29, 46, 56, 58, 50, 52, 33, 50, 42, 43, 52, 29, 56, 45, 69, 47, 30, 41, 55, 55, 54, 33, 46, 45, 66, 47, 51, 26, 57, 50, 46, 45, 43, 53, 60, 51, 33, 43, 61, 45, 55, 28, 52, 66, 42, 32, 42, 52, 61, 54, 47, 50, 46, 44, 56, 26, 52, 47, 75, 31, 46, 50, 57, 54, 34, 46, 46, 62, 42, 51, 28, 49, 72, 49, 44, 47, 54, 57, 52, 50, 32, 41, 69, 42, 54, 28, 66, 52, 46, 42, 56, 57, 55, 47, 33, 47, 44, 45, 51, 27, 53, 51, 69, 44, 28, 53, 59, 51, 35, 51, 62, 46, 54, 28, 51, 49, 68, 47, 42, 42, 56, 49, 31, 48, 66, 43, 56, 55, 74, 47, 43, 32, 45, 52, 56, 54, 49, 33, 49, 47, 43, 52, 29, 51, 48, 73, 42, 30, 46, 54, 50, 32, 47, 42, 64, 44, 54, 28, 54, 48, 68, 52, 46, 43, 53, 57, 46, 35, 45, 44, 50, 26, 56, 69, 45, 47, 30, 45, 52, 59, 52, 34, 51, 41, 45, 57, 27, 50, 50, 66, 43, 31, 42, 55, 63, 31, 51, 44, 65, 54, 27, 52, 48, 73, 46, 43, 46, 53, 55, 55, 51, 46, 60, 46, 50, 29, 51, 74, 50, 44, 29, 44, 54, 56, 52, 51, 32, 43, 43, 28, 55, 46, 70, 45, 31, 42, 56, 56, 52, 33, 48, 65, 44, 51, 27, 57, 50, 70, 49, 45, 43, 50, 50, 50, 34, 42, 60, 46, 57, 27, 50, 68, 49, 42, 31, 44, 53, 61, 55, 33, 49, 46, 42, 55, 26, 55, 47, 71, 44, 33, 47, 51, 55, 55, 33, 46, 45, 64, 52, 50, 47, 70, 52, 43, 45, 57, 60, 52, 50, 32, 42, 68, 42, 29, 54, 68, 51, 44, 29, 43, 57, 55, 52, 49, 35, 47, 45, 47, 50, 27, 50, 46, 29, 43, 49, 59, 52, 34, 50, 42, 63, 46, 55, 52, 49, 69, 48, 42, 42, 55, 60, 54, 46, 31, 46, 62, 41, 57, 27, 72, 47, 43, 33, 46, 50, 57, 54, 51, 33, 45, 45, 45, 51, 28, 50, 73, 43, 29, 47, 55, 59, 52, 32, 49, 44, 67, 42, 52, 28, 56, 48, 50, 47, 44, 55, 55, 54, 45, 43, 67, 44, 53, 26, 54, 47, 47, 29, 43, 51, 62, 53, 50, 33, 52, 41, 46, 53, 28, 50, 52, 41, 31, 43, 54, 59, 55, 51, 45, 62, 43, 55, 27, 52, 47, 74, 47, 45, 50, 55, 56, 51, 33, 47, 63, 46, 52, 28, 52, 73, 41, 30, 45, 56, 58, 49, 50, 31, 50, 44, 41, 55, 28, 57, 46, 66, 45, 43, 54, 58, 51, 35, 46, 44, 67, 47, 52, 54, 71, 51, 60, 48, 35, 44, 61, 45, 54, 27, 52, 66, 43, 32, 42, 60, 57, 46, 33, 45, 41, 55, 27, 53, 46, 71, 45, 30, 44, 52, 57, 56, 32, 48, 45, 62, 44, 51, 29, 51, 50, 73, 49, 41, 47, 57, 50, 51, 33, 42, 66, 43, 51, 29, 54, 69, 49, 47, 42, 54, 54, 47, 33, 47, 45, 47, 52, 26, 56, 50, 72, 46, 30, 43, 52, 60, 50, 33, 52, 43, 61, 45, 56, 28, 51, 50, 67, 49, 42, 52, 61, 54, 48, 31, 64, 43, 56, 26, 52, 75, 48, 44, 30, 46, 50, 58, 55, 49, 46, 46, 43, 51, 28, 52, 50, 71, 30, 47, 56, 53, 32, 41, 67, 42, 54, 29, 55, 46, 65, 51, 47, 42, 56, 56, 54, 47, 34, 69, 45, 50, 27, 54, 70, 46, 45, 28, 52, 60, 50, 49, 36, 52, 43, 46, 53, 27, 51, 49, 70, 43, 31, 41, 53, 58, 56, 31, 49, 47, 43, 54, 55, 46, 74, 47, 44, 45, 51, 54, 50, 33, 46, 61, 52, 29, 53, 71, 52, 41, 30, 46, 54, 59, 50, 52, 32, 48, 41, 44, 28, 54, 48, 68, 45, 30, 43, 55, 58, 35, 45, 45, 67, 45, 50, 26, 56, 52, 68, 46, 46, 45, 52, 59, 53, 35, 42, 62, 45, 57, 50, 67, 50, 43, 31, 42, 54, 61, 55, 31, 52, 44, 42, 55, 27, 48, 73, 44, 30, 47, 51, 54, 55, 34, 49, 46, 61, 44, 51, 29, 51, 74, 50, 43, 44, 53, 57, 53, 51, 31, 68, 43, 53, 28, 56, 69, 51, 44, 31, 42, 57, 55, 53, 46, 34, 48, 44, 46, 53, 27, 56, 50, 44, 30, 45, 51, 61, 49, 49, 42, 61, 46, 57, 27, 50, 69, 43, 43, 51, 62, 55, 46, 32, 47, 65, 53, 26, 54, 72, 46, 46, 52, 54, 56, 50, 34, 45, 43, 51, 28, 50, 48, 70, 43, 29, 44, 56, 60, 52, 32, 50, 41, 67, 42, 52, 29, 47, 68, 50, 46, 43, 57, 55, 51, 48, 35, 66, 47, 51, 27, 56, 72, 45, 46, 30, 50, 60, 52, 50, 34, 49, 42, 47, 55, 27, 52, 50, 68, 42, 33, 41, 59, 54, 31, 51, 47, 62, 42, 27, 53, 46, 71, 48, 43, 46, 50, 57, 55, 51, 33, 44, 61, 44, 52, 28, 50, 74, 52, 43, 28, 47, 53, 52, 50, 32, 48, 43, 41, 52, 28, 57, 48, 68, 46, 30, 54, 55, 35, 46, 43, 68, 44, 53, 27, 53, 49, 69, 46, 44, 52, 60, 53, 34, 41, 63, 55, 28, 50, 67, 48, 42, 31, 44, 54, 59, 53, 47, 32, 51, 47, 43, 55, 27, 54, 46, 74, 45, 32, 45, 55, 56, 47, 47, 64, 45, 27, 52, 47, 75, 51, 41, 45, 57, 58, 49, 50, 31, 44, 64, 42, 54, 29, 57, 66, 52, 45, 31, 42, 53, 57, 54, 49, 34, 46, 46, 52, 26, 55, 51, 72, 29, 44, 50, 62, 51, 35, 50, 43, 61, 46, 54, 27, 52, 52, 67, 48, 43, 43, 60, 56, 46, 33, 45, 42, 56, 52, 71, 48, 45, 31, 44, 53, 56, 56, 51, 32, 48, 45, 50, 29, 50, 50, 73, 42, 29, 47, 55, 57, 49, 33, 50, 42, 66, 44, 29, 47, 69, 49, 46, 42, 54, 54, 54, 49, 33, 46, 68, 47, 51, 26, 56, 71, 47, 44, 29, 42, 52, 61, 51, 47, 34, 51, 43, 44, 56, 52, 65, 41, 32, 43, 52, 61, 55, 32, 49, 44, 64, 44, 57, 26, 47, 73, 47, 44, 47, 50, 56, 54, 51, 33, 46, 42, 51, 28, 53, 70, 50, 44, 29, 47, 55, 57, 52, 49, 33, 49, 42, 41, 54, 28, 54, 46, 66, 46, 30, 41, 56, 57, 54, 34, 47, 44, 68, 46, 49, 27, 54, 52, 46, 44, 45, 52, 59, 51, 49, 42, 60, 46, 54, 28, 51, 69, 44, 31, 41, 53, 60, 55, 48, 31, 50, 46, 44, 56, 26, 55, 74, 33, 45, 52, 57, 54, 32, 47, 46, 61, 44, 52, 29, 52, 49, 70, 51, 42, 45, 55, 58, 51, 51, 32, 42, 64, 43, 54, 28, 53, 70, 52, 43, 54, 57, 52, 45, 36, 47, 45, 45, 50, 56, 52, 70, 47, 29, 51, 53, 34, 51, 42, 65, 44, 56, 27, 51, 50, 66, 50, 43, 41, 62, 57, 47, 31, 45, 66, 42, 55, 27, 52, 72, 46, 43, 31, 47, 53, 55, 54, 52, 34, 47, 46, 46, 51, 29, 51, 47, 73, 43, 45, 54, 52, 31, 47, 43, 68, 43, 54, 28, 57, 46, 68, 51, 45, 42, 56, 57, 46, 34, 46, 65, 52, 27, 56, 70, 48, 44, 30, 50, 60, 49, 35, 50, 42, 47, 56, 27, 51, 52, 69, 42, 31, 43, 51, 62, 56, 33, 50, 47, 63, 41, 54, 26, 54, 48, 46, 46, 46, 55, 50, 44, 63, 44, 52, 28, 50, 73, 51, 42, 29, 45, 57, 59, 53, 49, 31, 41, 43, 52, 29, 53, 49, 67, 46, 30, 43, 57, 54, 53, 34, 49, 64, 47, 50, 27, 56, 49, 72, 46, 47, 43, 50, 59, 52, 49, 34, 43, 63, 46, 55, 27, 53, 68, 48, 42, 32, 42, 54, 54, 47, 31, 52, 46, 41, 56, 27, 54, 48, 72, 43, 32, 45, 50, 57, 54, 33, 46, 45, 60, 53, 28, 50, 50, 74, 52, 42, 47, 55, 59, 50, 33, 43, 68, 42, 28, 56, 65, 49, 46, 31, 44, 54, 55, 53, 35, 46, 43, 45, 53, 26, 55, 49, 68, 47, 28, 44, 52, 61, 51, 34, 52, 42, 63, 46, 54, 49, 68, 48, 41, 43, 55, 59, 54, 48, 33, 46, 63, 43, 27, 73, 47, 32, 45, 50, 56, 57, 52, 32, 46, 47, 44, 51, 28, 53, 75, 41, 29, 44, 56, 58, 49, 31, 50, 43, 65, 41, 55, 29, 56, 46, 67, 51, 45, 43, 54, 57, 53, 47, 43, 65, 47, 52, 26, 53, 48, 29, 44, 50, 60, 51, 47, 34, 50, 44, 45, 54, 27, 52, 51, 67, 43, 33, 44, 53, 58, 56, 33, 44, 65, 41, 57, 26, 51, 47, 72, 47, 46, 52, 57, 56, 51, 32, 44, 63, 43, 50, 29, 51, 74, 49, 41, 29, 46, 55, 58, 51, 51, 32, 50, 43, 52, 29, 55, 46, 67, 47, 41, 55, 54, 55, 34, 45, 44, 68, 47, 51, 26, 56, 49, 47, 44, 52, 61, 50, 48, 33, 61, 45, 56, 28, 52, 66, 50, 42, 32, 43, 53, 47, 32, 50, 45, 43, 55, 52, 48, 74, 44, 46, 51, 56, 54, 35, 45, 47, 44, 50, 27, 53, 50, 70, 50, 43, 46, 55, 53, 50, 42, 67, 42, 54, 29, 54, 66, 51, 47, 29, 41, 57, 58, 47, 34, 48, 43, 50, 27, 52, 70, 44, 29, 45, 52, 60, 50, 34, 51, 42, 61, 46, 54, 28, 51, 50, 68, 47, 43, 41, 52, 58, 56, 48, 31, 46, 65, 43, 26, 54, 75, 48, 44, 32, 51, 55, 54, 49, 49, 46, 43, 53, 29, 51, 50, 71, 42, 30, 45, 54, 59, 50, 32, 42, 66, 43, 54, 28, 54, 48, 70, 51, 45, 43, 54, 57, 54, 45, 34, 66, 45, 51, 26, 56, 68, 46, 46, 29, 46, 52, 58, 53, 48, 35, 41, 45, 57, 50, 49, 66, 43, 31, 42, 53, 62, 56, 31, 51, 45, 42, 54, 27, 53, 47, 72, 46, 44, 46, 55, 53, 52, 34, 46, 61, 50, 28, 75, 50, 43, 29, 44, 55, 57, 51, 52, 32, 47, 44, 44, 28, 57, 46, 69, 45, 31, 41, 56, 56, 52, 33, 48, 45, 66, 44, 51, 27, 57, 68, 47, 45, 44, 51, 63, 50, 50, 34, 41, 60, 48, 57, 51, 69, 50, 42, 31, 44, 53, 62, 55, 46, 32, 49, 46, 42, 54, 26, 48, 71, 45, 32, 46, 52, 55, 57, 34, 47, 63, 43, 52, 29, 50, 71, 52, 44, 45, 56, 59, 52, 51, 31, 42, 67, 42, 53, 28, 54, 49, 45, 29, 44, 55, 54, 53, 49, 35, 48, 44, 46, 50, 27, 55, 49, 47, 29, 43, 49, 60, 53, 34, 49, 44, 62, 46, 55, 27, 51, 51, 68, 42, 42, 55, 59, 55, 45, 31, 46, 64, 42, 57, 27, 54, 71, 47, 32, 46, 50, 54, 52, 33, 46, 45, 45, 53, 28, 50, 49, 73, 28, 47, 54, 61, 33, 48, 43, 67, 41, 52, 28, 56, 47, 67, 50, 46, 43, 55, 55, 54, 47, 35, 43, 66, 45, 52, 26, 67, 48, 47, 29, 53, 61, 52, 49, 34, 51, 41, 45, 54, 28, 51, 51, 69, 42, 31, 43, 60, 53, 32, 52, 45, 63, 44, 54, 27, 54, 46, 75, 46, 45, 45, 51, 55, 52, 32, 46, 64, 44, 50, 28, 74, 50, 43, 30, 44, 56, 51, 49, 31, 49, 43, 42, 54, 29, 57, 46, 66, 45, 31, 53, 56, 35, 46, 44, 65, 47, 53, 26, 53, 51, 72, 47, 46, 45, 50, 61, 52, 35, 43, 44, 53, 27, 53, 67, 48, 43, 32, 43, 60, 57, 46, 32, 50, 45, 41, 57, 26, 53, 47, 72, 44, 30, 45, 53, 56, 56, 47, 44, 64, 44, 50, 29, 50, 49, 73, 50, 42, 47, 56, 57, 50, 52, 32, 43, 66, 42, 53, 29, 55, 68, 50, 47, 30, 42, 54, 55, 54, 47, 34, 46, 47, 51, 26, 55, 49, 72, 44, 30, 43, 53, 50, 34, 51, 43, 60, 45, 56, 28, 52, 51, 66, 50, 42, 42, 52, 62, 54, 48, 32, 44, 43, 56, 26, 53, 74, 47, 45, 30, 46, 50, 58, 50, 34, 47, 46, 50, 28, 53, 50, 71, 43, 30, 47, 56, 57, 53, 32, 48, 41, 68, 28, 53, 47, 66, 51, 47, 41, 56, 57, 54, 34, 43, 67, 47, 50, 27, 54, 71, 46, 45, 29, 45, 52, 59, 50, 50, 35, 52, 42, 46, 54, 51, 50, 68, 44, 31, 42, 51, 59, 56, 31, 50, 46, 66, 43, 55, 26, 46, 74, 47, 42, 45, 52, 56, 54, 49, 47, 60, 43, 53, 29, 52, 71, 52, 41, 29, 46, 55, 59, 51, 51, 47, 41, 43, 55, 28, 55, 48, 67, 45, 30, 44, 53, 57, 53, 34, 45, 45, 68, 44, 51, 57, 51, 46, 47, 45, 51, 59, 52, 35, 42, 64, 27, 50, 67, 43, 31, 42, 54, 61, 56, 47, 32, 51, 46, 42, 54, 27, 52, 48, 72, 31, 46, 52, 55, 54, 34, 60, 45, 49, 29, 51, 48, 74, 49, 43, 45, 54, 57, 52, 52, 31, 43, 68, 44, 54, 28, 57, 70, 49, 45, 42, 57, 57, 52, 46, 33, 47, 44, 45, 52, 27, 56, 50, 68, 46, 30, 51, 61, 50, 34, 50, 42, 60, 47, 56, 27, 50, 51, 69, 50, 43, 43, 60, 55, 46, 33, 46, 41, 55, 26, 54, 72, 46, 45, 32, 46, 51, 55, 57, 50, 33, 48, 43, 51, 28, 51, 48, 72, 43, 28, 44, 56, 52, 31, 49, 42, 68, 52, 29, 54, 48, 66, 50, 44, 44, 56, 55, 48, 36, 43, 66, 47, 51, 27, 55, 71, 46, 46, 29, 44, 50, 58, 51, 33, 49, 44, 47, 27, 52, 49, 68, 42, 31, 41, 54, 62, 54, 32, 51, 47, 64, 41, 56, 27, 54, 47, 71, 42, 46, 50, 57, 54, 52, 45, 60, 45, 52, 28, 51, 74, 52, 43, 29, 46, 53, 60, 51, 50, 33, 43, 41, 52, 28, 56, 47, 66, 47, 30, 43, 56, 55, 54, 35, 48, 67, 45, 53, 54, 50, 69, 48, 46, 43, 52, 61, 52, 48, 33, 42, 64, 47, 28, 50, 67, 47, 42, 31, 43, 55, 58, 55, 47, 32, 52, 46, 44, 54, 27, 46, 75, 46, 32, 45, 50, 55, 56, 32, 46, 46, 52, 28, 53, 48, 75, 50, 42, 45, 56, 57, 51, 50, 31, 43, 65, 42, 29, 57, 51, 45, 30, 42, 54, 57, 52, 48, 35, 45, 43, 46, 52, 26, 53, 52, 45, 29, 50, 61, 51, 35, 50, 43, 62, 46, 54, 52, 67, 48, 43, 43, 54, 59, 56, 47, 32, 45, 66, 41, 56, 26, 70, 48, 46, 31, 46, 52, 58, 55, 50, 33, 48, 45, 50, 29, 50, 41, 29, 46, 57, 56, 50, 33, 49, 43, 65, 44, 52, 29, 55, 46, 68, 50, 46, 41, 54, 55, 55, 48, 34, 45, 68, 46, 50, 26, 57, 45, 29, 43, 53, 61, 50, 48, 33, 51, 43, 45, 57, 28, 53, 51, 67, 41, 32, 43, 52, 61, 54, 32, 50, 44, 64, 43, 56, 26, 51, 48, 74, 48, 47, 51, 56, 56, 49, 33, 47, 61, 44, 28, 51, 71, 50, 44, 30, 47, 54, 56, 52, 49, 33, 49, 41, 41, 54, 28, 53, 67, 46, 42, 56, 57, 55, 33, 48, 43, 68, 45, 51, 27, 54, 52, 71, 46, 45, 52, 60, 50, 49, 35, 43, 59, 46, 55, 28, 51, 68, 43, 42, 59, 57, 48, 31, 50, 46, 44, 55, 26, 55, 46, 74, 43, 32, 45, 52, 56, 54, 32, 47, 47, 61, 43, 52, 28, 53, 49, 71, 52, 41, 54, 50, 51, 32, 42, 66, 44, 54, 27, 54, 70, 52, 46, 30, 42, 55, 56, 46, 35, 46, 46, 45, 49, 26, 57, 51, 68, 47, 30, 44, 60, 52, 36, 50, 41, 63, 45, 56, 27, 51, 48, 66, 50, 43, 41, 55, 61, 55, 48, 31, 45, 65, 43, 55, 27, 52, 73, 45, 42, 31, 47, 53, 55, 54, 51, 48, 45, 46, 50, 51, 49, 74, 43, 29, 44, 55, 57, 53, 31, 44, 67, 43, 53, 28, 56, 46, 69, 51, 45, 42, 56, 51, 46, 34, 66, 44, 52, 27, 55, 70, 48, 45, 29, 44, 50, 60, 51, 50, 34, 50, 42, 46, 56, 27, 50, 52, 69, 43, 31, 43, 52, 61, 32, 49, 47, 41, 54, 26, 54, 48, 71, 46, 44, 47, 52, 54, 57, 49, 34, 44, 64, 53, 28, 50, 29, 46, 56, 59, 51, 31, 50, 42, 42, 29, 47, 68, 45, 29, 44, 56, 56, 53, 48, 44, 65, 47, 50, 27, 55, 49, 72, 46, 47, 42, 51, 58, 52, 50, 34, 43, 63, 47, 54, 52, 68, 50, 41, 33, 41, 54, 62, 55, 46, 32, 51, 46, 42, 56, 27, 46, 71, 44, 31, 46, 51, 57, 53, 47, 45, 60, 44, 52, 28, 50, 74, 51, 42, 47, 54, 60, 50, 49, 32, 42, 67, 42, 52, 28, 56, 65, 49, 46, 31, 43, 56, 54, 54, 46, 35, 44, 46, 53, 27, 54, 49, 46, 29, 43, 52, 61, 52, 34, 52, 41, 64, 45, 54, 28, 50, 52, 68, 42, 44, 53, 59, 55, 48, 32, 63, 43, 54, 27, 54, 75, 46, 31, 44, 49, 55, 56, 51, 33, 46, 47, 45, 52, 28, 51, 48, 74, 42, 29, 45, 56, 57, 51, 32, 50, 44, 65, 42, 55, 29, 56, 47, 65, 51, 44, 42, 53, 56, 52, 48, 34, 43, 67, 46, 52, 26, 55, 48, 46, 28, 62, 51, 47, 35, 50, 43, 45, 54, 27, 51, 51, 66, 43, 32, 43, 59, 55, 32, 50, 45, 65, 42, 56, 26, 53, 46, 72, 48, 44, 52, 58, 57, 51, 33, 44, 63, 50, 30, 51, 49, 42, 28, 46, 57, 50, 52, 32, 50, 42, 43, 52, 29, 55, 46, 70, 46, 31, 41, 55, 55, 34, 46, 45, 68, 47, 26, 56, 50, 71, 47, 45, 43, 52, 60, 50, 33, 44, 61, 45, 56, 28, 67, 49, 42, 32, 43, 51, 60, 54, 48, 32, 49, 44, 43, 57, 52, 48, 75, 44, 31, 47, 50, 56, 55, 46, 47, 62, 43, 50, 28, 52, 50, 72, 43, 46, 55, 58, 53, 49, 33, 42, 68, 41, 54, 54, 65, 52, 46, 29, 42, 56, 57, 55, 47, 34, 47, 45, 51, 27, 54, 52, 70, 44, 29, 45, 52, 59, 49, 35, 52, 43, 61, 46, 54, 28, 48, 69, 49, 43, 43, 52, 59, 56, 47, 32, 47, 43, 56, 26, 53, 74, 48, 43, 44, 52, 55, 54, 50, 32, 47, 47, 52, 29, 52, 71, 30, 45, 53, 60, 51, 32, 48, 41, 65, 43, 28, 55, 48, 69, 51, 43, 55, 58, 52, 47, 34, 44, 66, 45, 51, 26, 57, 70, 45, 46, 30, 52, 60, 52, 48, 35, 50, 41, 45, 55, 50, 50, 66, 44, 41, 55, 60, 57, 31, 52, 45, 65, 43, 54, 27, 48, 47, 43, 46, 52, 55, 54, 51, 34, 46, 60, 45, 50, 29, 51, 75, 50, 44, 29, 45, 54, 57, 52, 52, 31, 48, 43, 43, 52, 28, 57, 46, 69, 45, 31, 41, 55, 56, 52, 34, 47, 45, 66, 45, 53, 27, 56, 51, 48, 45, 45, 51, 60, 51, 50, 34, 41, 61, 47, 57, 27, 51, 68, 31, 43, 52, 62, 55, 46, 33, 49, 47, 41, 54, 26, 55, 48, 70, 31, 47, 51, 56, 56, 34, 47, 46, 64, 43, 52, 28, 50, 48, 73, 52, 43, 57, 58, 52, 51, 32, 41, 68, 43, 52, 29, 54, 67, 50, 45, 55, 55, 52, 48, 36, 48, 44, 46, 50, 27, 55, 49, 71, 47, 50, 59, 52, 33, 49, 43, 63, 47, 56, 27, 53, 49, 70, 48, 41, 43, 60, 54, 45, 31, 46, 63, 42, 56, 27, 53, 71, 47, 44, 32, 51, 57, 54, 50, 33, 46, 45, 45, 53, 28, 50, 49, 75, 42, 29, 53, 51, 32, 49, 43, 67, 42, 53, 28, 56, 49, 66, 49, 47, 43, 54, 47, 35, 43, 68, 44, 52, 26, 54, 69, 48, 46, 29, 43, 63, 53, 34, 52, 42, 46, 54, 28, 50, 52, 68, 41, 31, 43, 55, 59, 54



Real Quadratic Fields Average Tamagawa Products D < 10000


1.599, 1.719, 1.360, 1.822, 1.905, 1.952, 1.734, 1.583, 1.725, 1.844, 2.323, 2.022, 1.560, 1.966, 1.640, 1.704, 1.460, 1.847, 2.043, 2.545, 2.045, 1.659, 1.648, 1.583, 1.905, 2.479, 1.772, 1.971, 2.091, 1.572, 1.911, 1.380, 1.989, 2.615, 1.977, 1.695, 1.712, 1.556, 2.485, 1.864, 1.978, 1.571, 2.018, 1.752, 2.801, 1.746, 1.351, 1.789, 2.109, 1.925, 1.543, 1.703, 1.756, 1.717, 2.520, 2.092, 1.507, 2.051, 1.679, 2.826, 1.423, 1.786, 1.924, 2.689, 2.108, 1.610, 1.759, 1.614, 1.862, 2.440, 1.935, 1.988, 1.907, 1.727, 1.551, 1.768, 1.972, 2.742, 2.058, 1.682, 1.644, 1.754, 2.437, 1.697, 2.049, 1.613, 1.970, 1.544, 2.910, 1.701, 1.462, 2.109, 2.085, 1.705, 1.622, 1.621, 1.869, 2.549, 1.979, 1.558, 2.073, 1.526, 1.705, 1.304, 1.859, 2.663, 1.902, 1.777, 1.735, 1.569, 1.775, 2.458, 1.921, 1.897, 2.054, 1.780, 2.902, 1.679, 1.770, 1.348, 2.072, 2.763, 1.908, 1.589, 1.718, 1.669, 2.531, 1.819, 2.119, 1.450, 2.131, 1.595, 2.882, 1.638, 1.905, 1.480, 1.701, 1.907, 2.107, 1.521, 1.733, 1.612, 1.891, 2.426, 2.071, 1.441, 1.932, 1.741, 3.012, 1.947, 1.991, 2.821, 1.711, 1.659, 1.768, 1.754, 2.372, 1.707, 2.089, 1.899, 1.620, 2.945, 1.696, 1.781, 1.430, 2.039, 2.638, 2.126, 1.657, 1.547, 2.591, 1.773, 1.892, 1.498, 2.052, 1.607, 1.644, 1.934, 1.289, 2.067, 1.998, 1.664, 1.760, 1.651, 1.768, 2.506, 1.878, 1.630, 2.036, 1.707, 2.868, 1.662, 1.361, 1.673, 2.122, 2.766, 1.960, 1.626, 1.746, 1.686, 2.563, 1.840, 2.138, 2.077, 1.634, 2.927, 1.879, 1.424, 2.759, 2.059, 1.616, 1.717, 2.357, 1.913, 1.999, 1.470, 1.960, 1.738, 1.522, 1.417, 1.934, 1.917, 1.960, 1.690, 1.658, 1.692, 2.358, 2.128, 1.554, 1.952, 1.554, 2.984, 1.780, 1.496, 1.790, 2.052, 2.662, 2.149, 1.594, 1.604, 1.515, 1.917, 2.614, 1.689, 1.960, 2.095, 1.635, 3.032, 1.699, 1.844, 1.323, 2.048, 2.662, 1.883, 1.706, 1.793, 1.626, 1.847, 1.950, 1.621, 1.992, 1.721, 2.874, 1.731, 1.822, 1.282, 1.812, 2.043, 1.963, 1.656, 1.738, 1.689, 1.667, 2.616, 2.064, 1.418, 2.075, 1.669, 2.926, 1.546, 1.405, 1.730, 1.990, 2.693, 2.131, 1.582, 1.752, 1.652, 1.938, 2.422, 1.852, 2.002, 1.655, 3.039, 1.571, 1.706, 1.438, 1.973, 2.779, 1.760, 1.613, 1.743, 2.381, 1.800, 2.139, 1.606, 1.871, 1.543, 3.022, 1.767, 1.423, 1.805, 2.124, 2.039, 1.685, 1.603, 1.602, 1.929, 2.545, 1.890, 2.138, 1.591, 1.611, 1.372, 1.908, 1.953, 2.597, 1.871, 1.773, 1.580, 1.809, 2.431, 1.872, 1.964, 1.680, 2.907, 1.750, 1.876, 1.348, 2.068, 2.853, 2.007, 1.546, 1.668, 1.676, 2.613, 1.784, 2.126, 1.446, 2.077, 2.865, 1.835, 1.465, 1.771, 1.958, 2.087, 1.568, 1.784, 1.657, 1.826, 2.323, 2.039, 1.514, 1.909, 1.783, 3.048, 1.575, 1.927, 1.883, 2.822, 2.082, 1.741, 1.647, 1.722, 1.765, 2.433, 1.740, 2.053, 1.864, 1.573, 1.645, 1.795, 1.397, 2.146, 2.575, 2.132, 1.576, 1.640, 2.637, 1.706, 1.896, 1.540, 2.130, 1.589, 3.062, 1.878, 1.381, 1.873, 2.035, 1.930, 1.748, 1.732, 1.630, 1.720, 2.487, 1.973, 1.622, 1.948, 1.687, 2.938, 1.754, 1.291, 1.675, 2.092, 2.848, 1.891, 1.619, 1.680, 1.771, 2.519, 1.844, 2.061, 2.130, 1.668, 2.952, 1.581, 1.846, 1.478, 1.888, 2.696, 2.051, 1.587, 1.794, 1.598, 2.344, 1.888, 2.057, 1.408, 2.002, 1.710, 3.082, 1.758, 1.928, 2.057, 1.718, 1.581, 1.645, 2.433, 2.120, 1.563, 1.961, 1.581, 2.951, 1.765, 1.453, 2.148, 2.684, 2.031, 1.599, 1.685, 1.614, 1.827, 2.511, 1.699, 1.967, 2.054, 1.620, 3.044, 1.648, 1.948, 1.306, 2.613, 1.948, 1.771, 1.800, 1.553, 2.531, 1.939, 1.857, 1.544, 2.011, 1.696, 2.958, 1.670, 1.865, 1.322, 1.721, 2.111, 1.964, 1.573, 1.688, 1.761, 1.818, 2.616, 2.022, 1.471, 2.137, 1.649, 2.863, 1.592, 1.457, 1.694, 2.001, 2.095, 1.579, 1.749, 1.679, 1.846, 1.943, 2.047, 1.855, 1.674, 1.627, 1.671, 2.864, 1.758, 1.575, 1.719, 2.324, 1.774, 2.090, 1.604, 1.998, 1.630, 3.033, 1.666, 1.471, 1.862, 2.045, 2.074, 1.637, 1.558, 1.894, 2.551, 2.015, 1.517, 2.115, 1.541, 3.113, 1.660, 1.362, 1.869, 1.964, 2.657, 1.973, 1.672, 1.721, 1.547, 1.751, 2.535, 1.867, 1.988, 2.007, 1.762, 2.862, 1.774, 1.742, 1.342, 2.140, 2.845, 1.927, 1.540, 1.751, 2.534, 1.731, 1.518, 2.028, 1.700, 2.852, 1.592, 1.947, 1.388, 1.744, 1.867, 2.139, 1.623, 1.800, 1.866, 2.424, 1.978, 1.421, 1.911, 1.714, 1.556, 1.354, 1.913, 1.958, 2.781, 2.041, 1.706, 1.638, 1.749, 2.437, 1.710, 2.058, 1.984, 1.541, 2.958, 1.661, 1.735, 1.471, 2.154, 2.575, 2.106, 1.703, 1.591, 1.606, 2.579, 1.811, 1.938, 1.583, 2.047, 1.534, 3.134, 1.698, 1.853, 1.324, 2.031, 1.900, 1.726, 1.734, 1.559, 1.782, 1.907, 2.049, 1.746, 2.932, 1.655, 1.389, 1.785, 2.087, 2.770, 1.863, 1.617, 1.721, 1.693, 1.741, 2.553, 2.112, 2.162, 1.588, 2.921, 1.919, 1.480, 1.889, 2.793, 2.113, 1.568, 1.729, 1.656, 2.409, 1.816, 1.403, 1.767, 3.072, 1.641, 1.362, 1.898, 1.993, 1.989, 1.662, 1.677, 1.758, 1.756, 2.308, 2.070, 1.639, 1.880, 1.635, 2.974, 1.730, 1.443, 1.813, 2.039, 2.598, 2.158, 1.695, 1.651, 1.549, 1.836, 2.623, 1.796, 1.898, 2.068, 3.137, 1.629, 1.942, 1.288, 2.056, 2.579, 1.988, 1.653, 1.762, 1.606, 2.554, 1.815, 1.932, 1.618, 1.663, 2.872, 1.687, 1.799, 1.357, 1.732, 2.138, 1.896, 1.596, 1.645, 1.767, 1.718, 2.605, 2.158, 1.488, 2.050, 2.946, 1.612, 1.421, 1.746, 2.742, 2.083, 1.612, 1.739, 1.617, 1.930, 2.351, 1.909, 1.962, 1.964, 1.765, 3.142, 1.559, 1.714, 1.418, 1.856, 2.760, 1.723, 1.680, 1.693, 2.301, 1.724, 2.154, 1.562, 2.006, 1.566, 1.772, 1.754, 1.445, 1.761, 2.041, 2.120, 1.624, 1.601, 1.536, 1.886, 2.635, 1.967, 1.490, 2.102, 1.632, 3.063, 1.303, 1.925, 2.057, 2.695, 1.930, 1.695, 1.778, 1.613, 1.704, 2.439, 1.852, 1.913, 1.996, 1.765, 2.850, 1.335, 2.066, 2.824, 1.942, 1.622, 1.723, 1.662, 2.598, 1.887, 2.086, 1.415, 2.028, 1.606, 2.948, 1.539, 1.949, 1.446, 1.729, 1.998, 2.104, 1.557, 1.772, 1.709, 1.908, 2.450, 1.941, 1.499, 1.989, 1.646, 3.068, 1.559, 1.819, 1.985, 2.796, 2.014, 1.564, 1.769, 1.817, 2.352, 1.766, 2.128, 1.911, 1.582, 3.070, 1.754, 1.725, 1.405, 2.119, 2.675, 2.053, 1.671, 1.591, 1.610, 2.525, 1.802, 1.857, 1.536, 2.133, 1.608, 1.584, 1.807, 1.377, 1.914, 1.910, 1.751, 1.792, 1.541, 1.744, 2.407, 1.992, 1.551, 2.077, 1.693, 2.884, 1.747, 1.346, 1.722, 2.016, 2.895, 1.978, 1.562, 1.650, 1.680, 1.748, 2.636, 1.752, 2.148, 2.079, 1.677, 2.865, 1.599, 1.837, 1.973, 2.060, 1.559, 1.799, 1.701, 2.351, 1.880, 2.008, 1.472, 1.855, 1.767, 3.067, 1.614, 1.761, 1.951, 1.885, 1.732, 1.692, 1.660, 1.803, 2.453, 2.038, 1.567, 1.864, 1.579, 3.052, 1.709, 1.399, 2.108, 2.551, 2.126, 1.631, 1.650, 1.950, 2.623, 1.678, 1.932, 2.159, 1.534, 3.074, 1.611, 1.873, 1.338, 2.039, 2.574, 1.943, 1.779, 1.729, 1.593, 2.515, 1.893, 1.992, 1.613, 1.968, 1.708, 2.925, 1.727, 1.745, 1.308, 1.712, 1.925, 1.606, 1.709, 1.783, 2.523, 2.061, 1.477, 2.152, 1.664, 2.947, 1.581, 1.470, 1.743, 1.938, 2.684, 2.056, 1.570, 1.801, 1.932, 2.294, 1.883, 2.065, 1.938, 1.685, 3.108, 1.618, 1.810, 1.432, 1.901, 2.867, 2.043, 1.671, 1.699, 2.467, 1.703, 2.109, 1.533, 1.980, 1.624, 2.989, 1.736, 1.471, 1.852, 2.104, 2.034, 1.621, 1.645, 1.633, 1.869, 2.495, 1.929, 1.532, 2.038, 1.630, 3.091, 1.637, 1.312, 1.901, 1.997, 1.971, 1.747, 1.814, 1.581, 1.681, 1.951, 1.850, 1.944, 1.734, 2.965, 1.684, 1.844, 1.322, 2.147, 2.777, 1.990, 1.550, 1.681, 1.719, 2.595, 2.082, 1.502, 2.160, 1.623, 2.831, 1.546, 1.894, 1.473, 1.726, 1.954, 1.608, 1.706, 1.691, 1.805, 2.408, 1.505, 1.887, 1.669, 1.339, 1.861, 1.967, 2.868, 1.760, 1.579, 1.854, 2.337, 1.790, 2.080, 1.986, 1.622, 3.049, 1.705, 1.697, 1.477, 2.024, 2.556, 2.059, 1.685, 1.537, 2.541, 1.694, 1.932, 2.143, 1.547, 3.104, 1.717, 1.920, 1.372, 1.952, 2.001, 1.692, 1.744, 1.564, 1.773, 2.519, 1.977, 1.556, 1.744, 2.863, 1.777, 1.312, 1.784, 2.135, 2.876, 1.852, 1.543, 1.746, 1.729, 1.704, 2.559, 1.742, 2.103, 2.062, 2.846, 1.577, 1.887, 1.402, 1.915, 2.745, 2.147, 1.639, 1.776, 1.602, 2.451, 1.941, 1.968, 1.455, 1.927, 1.682, 3.150, 1.571, 1.794, 1.896, 1.985, 2.060, 1.686, 1.728, 2.426, 2.074, 1.624, 1.944, 1.560, 1.666, 1.496, 1.800, 2.139, 2.545, 2.091, 1.697, 1.602, 1.620, 1.806, 2.583, 1.791, 1.970, 2.060, 1.552, 1.850, 1.306, 2.005, 2.674, 1.878, 1.706, 2.389, 1.910, 1.866, 1.594, 2.033, 1.787, 2.984, 1.683, 1.329, 1.763, 2.073, 1.914, 1.557, 1.747, 1.720, 1.757, 2.525, 2.109, 1.424, 2.125, 1.644, 2.930, 1.613, 1.494, 1.701, 1.878, 2.749, 2.146, 1.579, 1.705, 1.605, 2.403, 1.842, 2.073, 1.930, 1.762, 3.065, 1.744, 1.966, 2.884, 1.987, 1.645, 1.649, 1.782, 2.350, 1.704, 2.107, 1.632, 1.876, 1.589, 2.965, 1.706, 1.798, 1.409, 2.077, 2.140, 1.662, 1.645, 1.548, 1.879, 2.634, 1.929, 1.458, 2.043, 1.606, 3.159, 1.616, 1.341, 1.892, 2.552, 1.971, 1.670, 1.777, 1.595, 1.770, 2.569, 1.836, 1.879, 2.047, 1.679, 2.849, 1.683, 1.806, 1.341, 2.126, 2.765, 1.954, 1.634, 1.685, 1.777, 1.828, 2.156, 1.477, 2.093, 1.605, 2.958, 1.635, 1.858, 1.400, 1.706, 2.015, 1.646, 1.740, 1.626, 1.931, 2.333, 1.948, 1.461, 2.009, 1.765, 3.163, 1.565, 1.401, 1.902, 1.887, 2.791, 1.735, 1.669, 1.657, 1.881, 2.122, 1.964, 1.554, 2.988, 1.778, 1.740, 1.472, 2.079, 2.676, 2.106, 1.611, 1.543, 2.610, 1.729, 2.008, 1.457, 2.057, 1.607, 3.067, 1.691, 1.851, 1.350, 1.949, 2.077, 1.847, 1.699, 1.787, 1.636, 1.679, 2.451, 1.621, 2.012, 1.721, 2.852, 1.684, 1.314, 1.779, 2.024, 2.832, 1.966, 1.628, 1.695, 1.706, 2.634, 1.809, 2.030, 2.052, 1.664, 2.961, 1.550, 1.929, 1.417, 1.985, 2.667, 2.162, 1.533, 1.772, 2.396, 1.863, 1.975, 1.520, 1.966, 1.701, 3.104, 1.540, 1.726, 1.411, 1.995, 2.041, 1.775, 1.566, 1.760, 2.357, 2.130, 1.628, 1.896, 1.571, 3.068, 1.732, 1.417, 1.774, 2.081, 2.696, 2.095, 1.660, 1.606, 1.884, 2.572, 1.757, 1.893, 2.129, 1.595, 1.618, 1.877, 1.357, 1.970, 2.522, 1.862, 1.712, 1.774, 1.545, 1.917, 2.004, 1.540, 2.018, 1.684, 2.908, 1.763, 1.843, 1.379, 1.691, 2.052, 1.985, 1.540, 1.679, 1.693, 1.745, 2.648, 2.104, 1.462, 1.663, 2.820, 1.646, 1.439, 1.773, 1.976, 2.773, 2.066, 1.564, 1.799, 1.700, 1.862, 2.284, 1.835, 1.933, 1.751, 3.081, 1.591, 1.744, 1.357, 1.900, 2.858, 2.018, 1.787, 1.667, 1.655, 2.473, 1.763, 1.534, 1.912, 3.058, 1.658, 1.734, 1.384, 1.829, 2.161, 2.155, 1.638, 1.610, 1.606, 1.930, 2.615, 1.884, 2.159, 1.561, 3.050, 1.637, 1.367, 1.814, 2.062, 2.596, 1.914, 1.742, 1.751, 1.605, 1.715, 2.446, 1.929, 1.983, 1.638, 2.936, 1.776, 1.780, 1.325, 2.100, 2.855, 1.906, 1.642, 1.677, 2.549, 1.864, 2.030, 1.442, 2.131, 2.957, 1.556, 1.873, 1.488, 1.789, 1.873, 2.016, 1.570, 1.791, 1.599, 1.946, 2.327, 2.062, 1.403, 1.980, 1.690, 1.628, 1.416, 1.845, 1.882, 2.878, 2.068, 1.653, 1.600, 1.712, 1.808, 2.424, 1.733, 2.132, 1.938, 1.631, 1.713, 1.708, 1.455, 2.137, 2.646, 2.064, 1.639, 1.636, 1.593, 2.522, 1.686, 1.961, 1.565, 2.063, 1.642, 3.051, 1.927, 1.304, 1.941, 1.935, 2.002, 1.716, 1.793, 1.558, 1.683, 2.532, 1.939, 1.582, 1.952, 1.706, 2.995, 1.696, 1.285, 1.744, 2.161, 2.750, 1.962, 1.535, 1.664, 1.775, 1.807, 2.627, 1.795, 2.054, 2.103, 1.650, 2.863, 1.570, 1.475, 1.946, 2.654, 2.115, 1.599, 1.740, 1.671, 2.415, 1.902, 2.042, 1.506, 1.891, 1.703, 3.167, 1.616, 1.824, 1.948, 1.788, 1.602, 1.752, 2.295, 2.073, 1.983, 1.605, 3.091, 1.703, 1.469, 2.059, 2.565, 2.027, 1.649, 1.685, 1.553, 1.901, 2.539, 1.741, 1.969, 2.151, 1.548, 3.110, 1.672, 1.927, 1.346, 2.693, 1.995, 1.675, 1.702, 1.549, 2.529, 1.873, 1.948, 1.559, 2.035, 1.747, 2.822, 1.751, 1.736, 1.733, 2.164, 1.868, 1.562, 1.736, 1.720, 1.689, 2.531, 2.095, 1.469, 2.059, 1.654, 2.845, 1.568, 1.404, 1.809, 1.930, 2.136, 1.647, 1.801, 1.631, 1.830, 2.447, 1.936, 1.965, 1.926, 1.715, 3.184, 1.545, 1.803, 1.944, 2.797, 1.694, 1.627, 1.761, 2.397, 1.675, 2.008, 1.627, 1.557, 2.987, 1.701, 1.759, 1.477, 1.751, 2.156, 2.120, 1.628, 1.623, 1.827, 2.562, 1.939, 1.565, 2.031, 1.571, 3.180, 1.690, 1.302, 1.845, 2.624, 1.893, 1.768, 1.724, 1.577, 1.780, 2.430, 1.902, 1.939, 2.044, 1.755, 2.940, 1.672, 1.780, 1.362, 2.020, 2.815, 1.920, 1.559, 1.710, 2.559, 1.789, 2.151, 1.464, 2.124, 1.594, 2.915, 1.941, 1.462, 1.732, 1.909, 2.139, 1.549, 1.698, 1.873, 2.479, 2.088, 1.414, 1.899, 1.773, 3.064, 1.638, 1.395, 1.952, 1.945, 2.865, 1.991, 1.660, 1.687, 1.715, 2.324, 1.707, 2.103, 1.859, 2.954, 1.743, 1.788, 1.398, 2.053, 2.142, 1.686, 1.673, 1.573, 2.598, 1.742, 1.893, 1.492, 2.062, 1.585, 1.621, 1.902, 1.292, 1.890, 2.016, 1.988, 1.692, 1.781, 1.619, 1.758, 1.863, 1.596, 2.085, 1.716, 2.832, 1.650, 1.375, 1.734, 2.135, 2.785, 1.637, 1.626, 1.737, 1.737, 2.551, 2.126, 2.073, 1.605, 2.961, 1.627, 1.837, 1.439, 1.941, 2.784, 2.021, 1.589, 1.750, 1.652, 1.957, 1.466, 1.949, 1.721, 3.158, 1.559, 1.434, 1.943, 1.919, 1.655, 1.694, 1.842, 2.332, 2.137, 1.526, 1.996, 1.548, 3.032, 1.734, 1.493, 1.733, 2.063, 2.697, 2.108, 1.623, 1.555, 1.551, 1.877, 2.610, 1.711, 1.964, 2.106, 1.622, 3.100, 1.695, 1.842, 1.328, 2.077, 2.693, 1.894, 1.685, 1.810, 1.653, 2.404, 1.850, 1.920, 1.631, 1.765, 2.847, 1.723, 1.826, 1.315, 1.737, 2.043, 1.997, 1.631, 1.721, 1.648, 1.704, 2.594, 2.073, 1.467, 2.076, 2.937, 1.540, 1.423, 1.728, 1.961, 2.661, 2.154, 1.543, 1.708, 1.923, 2.470, 1.861, 1.959, 1.937, 1.673, 3.082, 1.544, 1.744, 1.390, 2.013, 2.743, 1.980, 1.741, 1.597, 1.737, 2.421, 1.785, 2.161, 1.594, 1.883, 1.548, 1.785, 1.688, 1.421, 1.805, 2.054, 2.052, 1.660, 1.596, 1.956, 2.570, 1.881, 1.558, 2.131, 1.612, 3.157, 1.326, 1.915, 1.936, 2.520, 1.907, 1.747, 1.805, 1.561, 1.782, 2.421, 1.853, 1.997, 2.059, 1.672, 2.911, 1.746, 1.357, 2.034, 2.901, 1.964, 1.567, 1.692, 1.655, 2.629, 1.771, 2.138, 1.425, 2.121, 1.715, 2.832, 1.631, 1.805, 1.419, 1.777, 2.008, 2.080, 1.579, 1.780, 1.680, 1.871, 2.330, 1.977, 1.516, 1.892, 1.752, 3.068, 1.577, 1.895, 1.908, 2.864, 2.047, 1.722, 1.673, 1.671, 1.750, 2.430, 1.770, 2.056, 1.881, 1.575, 3.060, 1.798, 1.436, 2.138, 2.528, 2.118, 1.646, 1.611, 1.645, 2.644, 1.724, 1.906, 1.528, 2.145, 1.528, 3.100, 1.605, 1.918, 1.374, 1.922, 1.724, 1.644, 1.715, 1.948, 1.611, 1.961, 1.675, 2.961, 1.779, 1.316, 1.708, 2.126, 2.895, 1.906, 1.606, 1.663, 1.714, 1.759, 2.508, 1.865, 2.130, 1.720, 2.973, 1.534, 1.802, 1.498, 1.901, 2.066, 1.598, 1.778, 1.587, 2.314, 2.055, 1.439, 2.008, 1.694, 3.122, 1.584, 1.785, 1.408, 1.886, 1.901, 1.676, 1.586, 1.698, 1.802, 2.424, 2.158, 1.550, 1.926, 1.603, 2.975, 1.756, 1.424, 1.844, 2.130, 2.671, 2.023, 1.663, 1.602, 1.885, 2.525, 1.717, 2.033, 1.610, 3.076, 1.683, 1.898, 1.332, 1.930, 2.584, 2.007, 1.746, 1.812, 1.551, 2.555, 1.923, 1.881, 1.542, 1.934, 1.740, 2.940, 1.712, 1.870, 1.292, 1.727, 2.134, 1.963, 1.563, 1.760, 1.787, 2.618, 2.094, 1.483, 2.150, 1.582, 2.872, 1.564, 1.475, 1.732, 1.932, 2.707, 2.049, 1.620, 1.731, 1.858, 2.431, 1.890, 2.066, 1.931, 1.675, 3.155, 1.694, 1.336, 1.968, 2.883, 2.017, 1.773, 1.559, 1.703, 2.329, 1.763, 2.056, 1.985, 1.625, 3.041, 1.684, 1.697, 1.498, 1.830, 2.060, 2.041, 1.612, 1.679, 1.544, 1.930, 2.495, 1.984, 1.487, 2.119, 1.556, 3.126, 1.690, 1.370, 1.836, 1.999, 2.642, 1.981, 1.692, 1.724, 1.566, 1.720, 1.862, 1.942, 1.751, 2.884, 1.719, 1.809, 1.332, 2.101, 2.899, 1.892, 1.559, 1.718, 1.777, 2.519, 2.066, 1.475, 2.051, 1.718, 2.869, 1.596, 1.961, 1.399, 1.772, 1.897, 2.145, 1.625, 1.808, 1.630, 1.816, 2.385, 1.445, 1.858, 1.535, 1.379, 1.876, 1.988, 2.744, 2.043, 1.675, 1.630, 1.756, 1.801, 2.411, 1.715, 2.047, 1.987, 1.570, 2.928, 1.676, 1.760, 2.128, 2.591, 2.116, 1.661, 1.568, 1.622, 2.600, 1.781, 1.994, 2.041, 1.556, 3.183, 1.640, 1.842, 1.291, 1.856, 2.055, 1.875, 1.747, 1.700, 1.574, 1.789, 2.477, 1.885, 1.774, 2.971, 1.701, 1.370, 1.803, 2.044, 2.765, 1.928, 1.569, 1.738, 1.688, 1.775, 2.548, 1.782, 2.134, 2.138, 1.653, 1.960, 1.453, 1.886, 2.764, 2.121, 1.569, 1.762, 1.620, 2.380, 1.806, 2.063, 1.446, 1.958, 1.712, 3.091, 1.646, 1.680, 1.385, 1.931, 1.937, 1.699, 1.685, 1.742, 1.770, 2.380, 2.098, 1.599, 1.894, 1.643, 1.407, 2.068, 2.613, 2.154, 1.691, 1.661, 1.538, 1.864, 2.628, 1.780, 1.880, 2.071, 1.577, 3.181, 1.893, 1.328, 2.061, 2.605, 1.939, 1.680, 1.758, 1.599, 2.522, 1.855, 1.919, 1.605, 2.057, 1.659, 2.824, 1.687, 1.354, 1.729, 2.139, 1.921, 1.644, 1.643, 1.755, 1.686, 2.611, 2.143, 1.504, 2.041, 1.604, 2.977, 1.421, 1.704, 2.805, 2.056, 1.619, 1.724, 1.656, 1.934, 2.280, 1.926, 1.968, 1.781, 1.587, 1.696, 1.929, 2.759, 2.002, 1.704, 1.659, 1.706, 2.280, 1.751, 2.113, 1.582, 1.949, 1.560, 3.038, 1.714, 1.772, 1.484, 2.160, 1.622, 1.556, 1.861, 2.630, 1.977, 1.501, 2.132, 1.647, 3.066, 1.670, 1.950, 2.658, 1.912, 1.677, 1.770, 1.646, 1.691, 2.431, 1.839, 1.969, 1.963, 1.717, 2.881, 1.678, 1.862, 1.303, 2.085, 2.793, 1.930, 1.588, 1.719, 1.697, 2.656, 1.870, 2.056, 1.420, 2.008, 1.646, 2.954, 1.566, 1.914, 1.444, 1.985, 2.173, 1.541, 1.766, 1.653, 1.943, 2.438, 1.946, 1.486, 1.975, 1.684, 3.046, 1.561, 1.414, 1.815, 1.967, 2.768, 1.779, 1.592, 1.757, 1.783, 2.385, 1.789, 2.137, 1.924, 1.546, 3.097, 1.756, 1.677, 1.381, 2.704, 2.041, 1.631, 1.576, 2.528, 1.758, 1.899, 1.510, 2.152, 3.162, 1.604, 1.851, 1.351, 1.912, 1.991, 1.876, 1.742, 1.797, 1.536, 1.793, 2.399, 1.929, 1.573, 2.082, 1.680, 2.872, 1.788, 1.367, 1.693, 2.075, 2.884, 1.966, 1.563, 1.678, 1.737, 2.619, 1.788, 2.155, 2.068, 1.684, 2.812, 1.633, 1.864, 1.439, 2.001, 2.744, 2.026, 1.543, 1.809, 2.378, 1.833, 1.989, 1.488, 1.897, 1.738, 3.112, 1.590, 1.782, 1.374, 1.906, 1.851, 2.022, 1.626, 1.709, 2.437, 2.050, 1.540, 1.927, 1.573, 3.069, 1.689, 1.382, 1.789, 2.164, 2.168, 1.621, 1.645, 1.607, 1.904, 2.619, 1.695, 1.901, 2.113, 1.577, 3.076, 1.602, 1.860, 1.390, 2.046, 2.521, 1.742, 1.717, 1.586, 1.937, 2.012, 1.644, 1.987, 1.711, 2.966, 1.754, 1.775, 1.315, 1.717, 2.085, 1.916, 1.598, 1.639, 1.771, 2.523, 2.060, 1.481, 2.124, 1.680, 2.984, 1.530, 1.459, 1.774, 1.904, 2.657, 2.049, 1.774, 1.619, 1.939, 2.368, 1.878, 1.963, 1.713, 3.148, 1.643, 1.773, 1.427, 1.852, 2.864, 2.053, 1.676, 1.597, 1.679, 2.434, 1.710, 2.129, 1.564, 1.912, 1.598, 2.962, 1.764, 1.438, 1.839, 2.129, 1.618, 1.677, 1.645, 1.842, 2.505, 1.956, 2.044, 1.603, 3.097, 1.683, 1.309, 1.936, 1.966, 2.632, 1.953, 1.765, 1.798, 1.535, 1.712, 2.514, 1.932, 1.902, 1.745, 2.926, 1.646, 1.804, 1.299, 2.161, 2.811, 1.972, 1.583, 1.738, 2.649, 1.799, 2.014, 1.504, 2.163, 2.835, 1.565, 1.845, 1.490, 1.697, 2.000, 2.090, 1.619, 1.753, 1.686, 1.842, 2.328, 2.084, 1.477, 1.895, 1.672, 3.158, 1.619, 1.846, 1.935, 2.863, 1.946, 1.772, 1.595, 1.858, 2.342, 1.797, 2.015, 2.001, 1.590, 1.659, 1.714, 1.502, 2.019, 2.563, 2.066, 1.656, 1.570, 2.540, 1.738, 1.942, 1.459, 2.132, 1.563, 3.140, 1.937, 1.333, 1.857, 1.989, 1.986, 1.663, 1.750, 1.555, 2.531, 1.984, 1.555, 1.965, 1.757, 2.881, 1.730, 1.329, 1.758, 2.128, 2.875, 1.918, 1.561, 1.705, 1.765, 1.695, 2.500, 1.756, 2.124, 2.075, 1.682, 2.810, 1.562, 1.957, 1.413, 1.896, 2.740, 2.150, 1.601, 1.776, 1.635, 2.462, 1.917, 1.982, 1.471, 1.868, 1.727, 3.183, 1.539, 1.750, 1.918, 1.986, 2.053, 1.652, 1.633, 1.741, 2.457, 2.085, 1.615, 1.950, 1.583, 2.960, 1.690, 1.481, 2.141, 2.525, 2.126, 1.673, 1.594, 1.610, 1.869, 1.742, 1.937, 2.008, 1.570, 3.176, 1.693, 1.886, 1.294, 2.668, 1.920, 1.762, 1.734, 1.610, 2.421, 1.905, 1.910, 1.567, 2.087, 1.736, 2.992, 1.787, 1.349, 1.790, 2.033, 1.875, 1.608, 1.740, 1.680, 1.768, 2.536, 2.152, 1.408, 2.137, 1.615, 2.897, 1.471, 1.697, 1.901, 2.124, 1.550, 1.724, 1.606, 1.882, 2.444, 1.873, 2.020, 1.951, 1.728, 3.048, 1.639, 1.709, 1.408, 2.003, 2.901, 1.662, 1.675, 1.715, 2.297, 1.724, 1.587, 1.901, 1.620, 2.922, 1.711, 1.783, 1.443, 1.868, 2.093, 2.111, 1.554, 1.816, 2.656, 1.849, 1.474, 2.087, 1.566, 1.600, 1.310, 1.870, 2.041, 2.599, 1.945, 1.682, 1.770, 1.634, 1.791, 2.483, 1.812, 1.896, 2.065, 1.696, 2.851, 1.722, 1.828, 1.335, 2.138, 2.790, 1.928, 1.625, 1.773, 2.537, 1.858, 2.122, 1.521, 2.035, 1.624, 2.987, 1.615, 1.825, 1.436, 1.675, 1.922, 2.080, 1.658, 1.715, 1.904, 2.306, 1.978, 1.998, 1.769, 3.153, 1.552, 1.412, 1.953, 1.896, 2.789, 1.959, 1.703, 1.652, 1.681, 2.383, 1.706, 2.159, 1.946, 1.536, 3.055, 1.760, 1.754, 1.469, 2.058, 2.649, 2.102, 1.600, 1.557, 2.650, 1.727, 2.010, 1.493, 1.628, 3.076, 1.674, 1.837, 1.331, 1.943, 2.049, 1.928, 1.658, 1.796, 1.602, 1.720, 1.924, 1.633, 1.919, 1.756, 2.821, 1.718, 1.312, 1.756, 2.031, 2.817, 1.991, 1.624, 1.756, 1.674, 1.713, 2.599, 2.066, 2.075, 2.995, 1.579, 1.912, 1.389, 1.954, 2.654, 2.140, 1.559, 1.758, 1.677, 2.443, 1.824, 1.490, 1.988, 1.710, 3.069, 1.529, 1.745, 1.399, 1.815, 1.967, 2.049, 1.765, 1.760, 1.770, 2.393, 2.105, 1.625, 1.921, 1.538, 3.073, 1.757, 1.437, 1.784, 2.100, 2.682, 2.010, 1.663, 1.609, 1.597, 2.495, 1.801, 1.926, 2.102, 1.601, 3.180, 1.600, 1.873, 1.376, 2.003, 2.517, 1.859, 1.722, 1.807, 1.586, 2.444, 1.903, 1.969, 1.536, 1.677, 1.749, 1.871, 1.382, 1.682, 2.054, 1.977, 1.543, 1.627, 1.682, 1.760, 2.606, 2.104, 1.420, 2.110, 2.848, 1.629, 1.442, 1.737, 1.989, 2.803, 2.072, 1.539, 1.799, 1.692, 1.800, 2.342, 1.882, 1.987, 1.892, 1.754, 3.098, 1.743, 1.919, 2.830, 2.077, 1.782, 1.674, 1.678, 2.376, 1.760, 2.091, 1.547, 1.907, 1.601, 1.678, 1.808, 1.402, 1.832, 2.107, 2.132, 1.601, 1.634, 1.621, 1.912, 2.632, 1.920, 1.571, 2.148, 1.534, 3.109, 1.355, 1.867, 2.047, 2.510, 1.925, 1.746, 1.734, 1.619, 1.732, 2.513, 1.954, 1.962, 1.946, 1.723, 2.941, 1.765, 1.319, 2.085, 2.861, 1.885, 1.604, 1.676, 1.675, 2.559, 1.810, 2.028, 1.451, 2.125, 1.680, 2.953, 1.568, 1.848, 1.774, 1.866, 2.038, 1.592, 1.805, 1.625, 1.962, 2.083, 1.450, 2.000, 1.651, 3.148, 1.632, 1.891, 1.868, 2.889, 2.061, 1.713, 1.585, 1.661, 1.772, 2.464, 1.698, 2.148, 1.921, 1.644, 2.934, 1.744, 1.688, 2.156, 2.677, 2.077, 1.618, 1.659, 1.588, 1.731, 1.946, 1.586, 2.078, 1.601, 3.061, 1.675, 1.884, 1.303, 1.886, 1.956, 1.750, 1.800, 1.559, 1.728, 2.503, 1.891, 1.556, 1.933, 1.701, 2.946, 1.690, 1.319, 2.149
2.763, 1.976, 1.557, 1.679, 1.783, 1.759, 2.652, 1.765, 2.027, 2.172, 1.602, 2.897, 1.536, 1.908, 1.490, 1.968, 2.058, 1.629, 1.690, 1.712, 2.358, 1.912, 2.037, 1.462, 1.873, 1.690, 1.626, 1.361, 1.735, 1.623, 1.823, 2.309, 2.019, 1.608, 1.956, 1.625, 3.090, 1.682, 1.490, 2.062, 2.547, 2.089, 1.629, 1.538, 1.931, 2.492, 1.982, 2.155, 1.576, 3.100, 1.653, 1.934, 1.366, 1.958, 2.698, 1.990, 1.695, 1.711, 1.557, 2.545, 1.823, 1.966, 1.583, 1.999, 1.715, 2.882, 1.714, 1.778, 1.320, 1.814, 2.167, 1.879, 1.538, 1.762, 1.709, 2.521, 2.127, 1.479, 2.055, 1.710, 2.831, 1.611, 1.418, 1.787, 1.863, 2.139, 1.629, 1.821, 1.862, 2.458, 1.897, 1.964, 1.895, 1.700, 3.164, 1.563, 1.762, 1.357, 1.941, 2.747, 2.069, 1.700, 1.644, 1.764, 2.442, 1.695, 2.059, 1.613, 1.967, 1.552, 2.970, 1.709, 1.742, 1.449, 1.783, 2.138, 1.678, 1.607, 1.609, 1.829, 2.615, 1.519, 2.064, 1.566, 3.171, 1.692, 1.295, 1.849, 2.026, 2.714, 1.900, 1.751, 1.704, 1.580, 1.812, 1.939, 1.903, 2.078, 1.718, 2.916, 1.696, 1.759, 1.364, 2.772, 1.885, 1.744, 1.650, 2.531, 2.172, 1.442, 2.105, 1.625, 2.872, 1.602, 1.912, 1.498, 1.734, 1.886, 2.128, 1.555, 1.748, 1.627, 1.868, 2.426, 1.419, 1.947, 1.767, 3.095, 1.608, 1.394, 1.902, 1.975, 2.899, 1.699, 1.636, 1.772, 1.795, 2.273, 1.690, 2.063, 1.905, 1.650, 3.006, 1.739, 1.796, 1.381, 2.043, 2.629, 2.159, 1.650, 1.687, 1.568, 2.633, 1.779, 1.862, 2.048, 1.607, 1.599, 1.922, 1.313, 1.874, 2.027, 1.978, 1.717, 1.621, 1.757, 2.493, 1.915, 1.616, 1.681, 2.835, 1.658, 1.367, 1.699, 2.142, 2.769, 1.938, 1.609, 1.656, 1.766, 1.684, 2.593, 1.847, 2.147, 2.032, 2.963, 1.607, 1.843, 1.424, 1.961, 2.771, 2.047, 1.591, 1.695, 2.348, 1.951, 1.984, 1.443, 1.979, 1.768, 3.179, 1.565, 1.679, 1.442, 1.923, 1.907, 1.978, 1.705, 1.668, 1.670, 2.356, 2.119, 1.575, 1.984, 1.542, 1.750, 1.451, 1.767, 2.058, 2.641, 2.132, 1.637, 1.606, 1.578, 2.611, 1.676, 2.005, 2.113, 1.588, 3.081, 1.841, 1.326, 2.027, 2.715, 1.881, 1.720, 1.822, 1.586, 2.434, 1.817, 1.909, 1.614, 2.007, 1.739, 2.831, 1.714, 1.308, 1.776, 2.047, 2.005, 1.650, 1.711, 1.665, 1.738, 2.653, 1.430, 2.044, 1.651, 2.925, 1.572, 1.416, 1.733, 2.002, 2.661, 2.117, 1.536, 1.789, 1.669, 1.927, 2.411, 1.847, 2.007, 1.926, 1.658, 3.084, 1.555, 1.754, 1.989, 2.774, 1.974, 1.738, 1.596, 1.788, 1.809, 2.116, 1.609, 1.907, 1.537, 3.085, 1.746, 1.419, 2.084, 2.043, 1.708, 1.577, 1.590, 1.939, 2.527, 1.892, 1.512, 1.655, 3.195, 1.608, 1.353, 1.938, 1.939, 1.675, 1.810, 1.551, 1.743, 2.388, 1.964, 2.042, 1.720, 2.950, 1.752, 1.828, 1.377, 2.051, 2.853, 2.016, 1.565, 1.630, 1.683, 2.600, 1.761, 2.148, 1.453, 2.113, 1.702, 2.821, 1.873, 1.443, 1.775, 1.937, 2.077, 1.532, 1.788, 1.712, 1.833, 2.362, 1.487, 1.875, 1.743, 3.112, 1.574, 1.350, 1.953, 1.901, 2.790, 1.744, 1.637, 1.695, 1.766, 2.432, 1.795, 2.095, 1.883, 1.589, 3.087, 1.681, 1.775, 1.438, 2.135, 2.515, 2.147, 1.653, 1.619, 2.640, 1.719, 1.861, 1.576, 2.114, 3.034, 1.643, 1.916, 1.365, 1.832, 2.037, 1.939, 1.762, 1.728, 1.602, 1.722, 2.443, 1.996, 1.609, 1.998, 1.685, 2.973, 1.762, 1.307, 1.696, 2.081, 2.913, 1.860, 1.639, 1.686, 1.743, 2.562, 1.856, 2.042, 2.148, 1.696, 2.954, 1.538, 1.823, 1.441, 1.929, 2.718, 1.613, 1.791, 2.304, 1.901, 2.060, 1.424, 2.004, 1.669, 3.107, 1.656, 1.783, 1.417, 1.897, 2.010, 1.684, 1.617, 1.655, 2.398, 2.145, 1.559, 1.594, 2.937, 1.757, 1.465, 1.832, 2.136, 2.642, 2.032, 1.638, 1.669, 1.639, 1.864, 2.574, 1.737, 1.883, 2.073, 1.601, 3.074, 1.637, 1.933, 1.313, 1.974, 2.599, 1.954, 1.793, 1.566, 1.877, 1.889, 1.530, 1.976, 3.005, 1.704, 1.860, 1.298, 1.733, 2.146, 1.984, 1.525, 1.691, 1.784, 1.771, 2.635, 2.034, 1.516, 2.124, 1.611, 2.864, 1.537, 1.483, 1.691, 1.985, 2.620, 2.124, 1.652, 1.713, 1.640, 1.819, 2.382, 1.915, 1.917, 1.696, 3.165, 1.598, 1.717, 1.349, 2.890, 2.007, 1.743, 1.577, 1.729, 2.354, 1.767, 2.084, 1.615, 1.939, 1.613, 3.092, 1.679, 1.702, 1.450, 1.848, 2.069, 2.058, 1.642, 1.567, 1.938, 2.515, 1.974, 2.102, 1.569, 1.673, 1.360, 1.855, 1.958, 2.677, 1.992, 1.654, 1.742, 1.548, 1.734, 2.555, 1.831, 1.943, 1.770, 2.833, 1.779, 1.778, 1.321, 2.111, 2.840, 1.863, 1.585, 1.735, 1.787, 2.498, 1.776, 2.128, 1.488, 2.038, 2.877, 1.901, 1.406, 1.793, 1.912, 2.119, 1.618, 1.817, 1.616, 1.816, 2.457, 1.939, 1.431, 1.893, 1.718, 3.162, 1.563, 1.365, 1.873, 1.991, 2.826, 2.089, 1.686, 1.595, 1.720, 1.874, 2.410, 1.724, 2.046, 2.002, 1.546, 1.688, 1.493, 2.165, 2.597, 2.083, 1.678, 1.596, 1.589, 2.554, 1.797, 1.989, 1.530, 2.038, 1.529, 3.186, 1.861, 1.321, 1.872, 2.034, 1.881, 1.775, 1.746, 1.606, 1.736, 2.454, 1.912, 2.093, 1.733, 2.973, 1.667, 1.377, 1.769, 2.004, 2.813, 1.857, 1.580, 1.736, 1.694, 1.804, 2.486, 1.786, 2.102, 2.152, 1.626, 2.926, 1.630, 1.941, 1.476, 1.907, 2.764, 2.162, 1.553, 1.736, 1.625, 2.414, 1.864, 2.022, 1.426, 1.913, 1.792, 3.091, 1.625, 1.690, 1.914, 1.988, 1.965, 1.677, 1.651, 1.727, 1.781, 2.124, 1.634, 1.909, 1.627, 2.957, 1.724, 1.410, 2.003, 2.668, 2.155, 1.658, 1.641, 1.580, 1.832, 2.657, 1.763, 1.933, 2.038, 1.570, 3.201, 1.604, 1.304, 2.511, 1.958, 1.682, 1.733, 1.614, 2.542, 1.861, 1.924, 1.620, 2.031, 1.705, 2.819, 1.674, 1.782, 1.381, 1.718, 2.109, 1.949, 1.603, 1.693, 1.726, 1.717, 2.582, 2.135, 1.526, 2.050, 1.611, 2.945, 1.653, 1.388, 1.688, 2.069, 1.616, 1.724, 1.680, 1.950, 2.294, 1.886, 1.979, 1.985, 1.757, 1.551, 1.704, 1.387, 1.861, 2.811, 1.720, 1.673, 2.387, 1.731, 2.118, 1.513, 2.000, 1.571, 3.018, 1.723, 1.766, 1.480, 1.777, 2.070, 2.155, 1.576, 1.541, 1.897, 2.633, 1.959, 1.482, 2.107, 1.604, 3.077, 1.686, 1.352, 1.910, 2.081, 2.665, 1.880, 1.659, 1.809, 1.612, 1.699, 2.419, 1.890, 1.926, 1.928, 1.731, 2.804, 1.727, 1.889, 1.323, 2.073, 1.968, 1.623, 1.693, 2.626, 1.858, 2.043, 1.422, 2.086, 1.635, 2.972, 1.539, 1.923, 1.428, 1.714, 1.985, 2.097, 1.560, 1.740, 1.927, 2.416, 1.938, 1.500, 1.688, 3.103, 1.564, 1.388, 1.852, 1.999, 2.779, 1.764, 1.627, 1.794, 2.347, 1.761, 2.136, 1.877, 1.567, 3.079, 1.735, 1.699, 1.422, 2.091, 2.673, 2.060, 1.708, 1.580, 1.556, 2.497, 1.763, 1.892, 1.547, 2.157, 1.629, 3.175, 1.626, 1.846, 1.926, 1.921, 1.930, 1.785, 1.768, 1.988, 1.560, 2.024, 1.677, 2.914, 1.745, 1.333, 1.725, 2.091, 2.857, 1.971, 1.530, 1.666, 1.670, 1.779, 2.653, 2.165, 2.049, 1.672, 2.854, 1.656, 1.814, 1.461, 1.936, 2.764, 2.066, 1.537, 1.809, 1.660, 2.369, 1.816, 1.513, 1.883, 1.753, 3.044, 1.573, 1.798, 1.342, 1.933, 1.876, 2.080, 1.767, 1.661, 1.684, 1.794, 2.408, 2.083, 1.550, 1.919, 1.594, 3.077, 1.667, 1.424, 1.840, 2.107, 2.583, 2.127, 1.636, 1.606, 1.897, 2.638, 1.700, 1.900, 2.163, 1.573, 3.072, 1.610, 1.839, 1.341, 2.073, 2.574, 1.956, 1.752, 1.715, 1.614, 2.477, 1.925, 1.956, 1.641, 1.665, 2.966, 1.751, 1.764, 1.303, 1.688, 2.108, 1.886, 1.597, 1.656, 1.757, 2.500, 2.067, 1.432, 2.126, 2.956, 1.564, 1.506, 1.799, 1.911, 2.617, 2.011, 1.614, 1.776, 1.646, 2.323, 1.920, 2.042, 1.982, 1.651, 3.157, 1.598, 1.796, 1.442, 1.886, 2.904, 2.025, 1.674, 1.600, 1.708, 2.433, 1.693, 2.116, 1.558, 1.923, 1.616, 1.780, 1.443, 1.827, 2.169, 2.085, 1.596, 1.666, 1.629, 1.840, 2.473, 1.917, 1.554, 2.045, 3.087, 1.321, 1.894, 2.600, 1.958, 1.779, 1.770, 1.531, 1.690, 2.528, 1.943, 1.896, 1.998, 1.715, 2.971, 1.667, 1.295, 2.142, 2.800, 1.994, 1.558, 1.695, 1.781, 2.640, 1.750, 2.061, 1.501, 2.148, 1.604, 2.869, 1.547, 1.906, 1.450, 1.707, 1.968, 2.078, 1.612, 1.711, 1.656, 1.880, 2.052, 1.489, 1.890, 1.692, 3.182, 1.640, 1.834, 2.840, 2.004, 1.756, 1.627, 1.709, 1.874, 2.365, 1.754, 2.004, 1.944, 1.630, 3.052, 1.706, 1.723, 1.452, 2.061, 2.518, 2.027, 1.652, 1.687, 1.554, 2.516, 1.996, 1.493, 2.144, 1.534, 3.167, 1.722, 1.894, 1.345, 1.883, 1.935, 1.679, 1.737, 1.551, 1.735, 2.563, 2.002, 1.548, 2.038, 1.764, 2.797, 1.727, 1.309, 1.794, 2.165, 2.893, 1.925, 1.576, 1.692, 1.720, 1.708, 2.564, 1.771, 2.050, 1.677, 2.804, 1.594, 1.906, 1.446, 1.876, 2.143, 1.592, 1.810, 1.598, 2.398, 1.948, 2.005, 1.432, 1.896, 1.708, 3.182, 1.559, 1.788, 1.883, 2.015, 1.702, 1.617, 1.764, 1.846, 2.440, 1.602, 1.964, 1.549, 2.990, 1.674, 1.477, 1.765, 2.091, 2.575, 2.072, 1.643, 1.859, 2.574, 1.744, 1.964, 2.077, 1.582, 1.692, 1.857, 1.311, 2.015, 1.915, 1.729, 1.745, 1.614, 2.366, 1.965, 1.879, 2.021, 1.756, 2.999, 1.649, 1.774, 1.385, 1.763, 2.051, 1.897, 1.601, 1.672, 1.773, 2.135, 1.452, 2.137, 1.627, 2.863, 1.618, 1.482, 1.706, 1.866, 2.807, 2.165, 1.528, 1.707, 1.890, 2.429, 1.857, 2.083, 1.754, 3.096, 1.693, 1.381, 1.989, 2.882, 1.947, 1.687, 1.632, 1.746, 2.370, 1.739, 2.107, 1.596, 1.898, 1.629, 2.981, 1.714, 1.744, 1.427, 1.875, 2.043, 2.147, 1.686, 1.677, 1.550, 1.837, 2.633, 1.902, 1.499, 2.044, 3.156, 1.633, 1.289, 1.844, 2.023, 2.570, 1.715, 1.782, 1.631, 1.806, 1.803, 1.904, 2.081, 1.667, 2.853, 1.721, 1.772, 1.363, 2.124, 2.784, 1.941, 1.626, 1.667, 1.753, 2.594, 2.135, 1.483, 2.073, 1.637, 2.921, 1.609, 1.822, 1.382, 1.711, 1.967, 2.049, 1.617, 1.725, 1.633, 1.948, 2.365, 1.475, 1.964, 1.724, 3.187, 1.564, 1.439, 1.907, 1.910, 2.798, 1.940, 1.694, 1.678, 1.669, 1.842, 2.329, 2.151, 1.968, 1.532, 1.744, 1.810, 1.475, 2.075, 2.633, 2.130, 1.654, 1.577, 1.552, 2.660, 1.709, 1.970, 2.089, 1.613, 3.081, 1.663, 1.869, 1.348, 1.922, 2.010, 1.903, 1.798, 1.637, 1.699, 2.380, 1.911, 1.619, 1.773, 2.896, 1.287, 1.750, 2.087, 2.828, 2.001, 1.595, 1.734, 1.713, 1.697, 2.601, 1.861, 2.016, 2.022, 2.989, 1.533, 1.929, 1.406, 1.970, 2.647, 2.163, 1.565, 1.759, 1.674, 2.439, 1.828, 1.971, 1.488, 2.000, 1.723, 3.068, 1.544, 1.427, 1.881, 1.959, 2.020, 1.741, 1.551, 1.766, 1.752, 2.410, 2.149, 1.627, 1.854, 1.534, 1.742, 1.412, 1.769, 2.123, 2.626, 2.028, 1.645, 1.589, 1.592, 1.919, 2.551, 1.792, 1.911, 2.123, 1.613, 3.174, 1.851, 1.371, 1.984, 2.557, 1.932, 1.702, 1.806, 1.535, 2.422, 1.863, 1.552, 2.040, 1.680, 2.850, 1.773, 1.365, 1.693, 2.031, 1.959, 1.570, 1.661, 1.694, 1.725, 2.621, 2.138, 1.442, 2.137, 1.662, 2.899, 1.608, 1.811, 1.978, 2.803, 2.028, 1.580, 1.823, 1.672, 1.810, 2.334, 1.824, 2.019, 1.926, 1.776, 3.038, 1.579, 1.781, 1.895, 2.859, 2.053, 1.785, 1.645, 1.649, 2.399, 1.787, 2.019, 1.581, 1.921, 1.576, 3.068, 1.708, 1.733, 1.428, 2.137, 2.127, 1.601, 1.662, 1.593, 1.946, 2.623, 1.904, 1.530, 2.102, 1.544, 3.053, 1.635, 1.366, 1.869, 2.527, 1.914, 1.770, 1.625, 1.696, 2.499, 1.934, 1.972, 1.960, 1.671, 2.995, 1.749, 1.782, 1.326, 2.911, 1.860, 1.611, 1.617, 2.507, 1.842, 2.065, 1.459, 2.161, 1.685, 2.966, 1.549, 1.879, 1.459, 1.758, 1.898, 2.074, 1.593, 1.804, 1.637, 1.900, 2.346, 2.044, 1.464, 1.959, 1.687, 3.135, 1.446, 1.845, 1.893, 2.861, 1.667, 1.593, 1.678, 1.792, 2.388, 1.716, 2.175, 1.953, 1.635, 2.969, 1.733, 1.709, 1.421, 2.139, 2.670, 2.072, 1.631, 1.659, 2.542, 1.678, 1.945, 1.564, 2.012, 1.622, 3.117, 1.621, 1.941, 1.296, 1.908, 1.985, 1.974, 1.734, 1.785, 1.702, 2.566, 1.899, 1.525, 1.988, 1.744, 2.971, 1.314, 1.769, 2.086, 2.733, 1.997, 1.556, 1.732, 1.801, 2.649, 1.780, 2.046, 2.103, 1.617, 2.826, 1.546, 1.920, 1.472, 1.957, 2.615, 1.638, 1.762, 2.352, 1.909, 2.037, 1.503, 1.880, 1.648, 3.202, 1.639, 1.708, 1.352, 1.867, 1.936, 1.954, 1.755, 1.615, 1.696, 2.314, 2.049, 2.007, 1.648, 3.042, 1.664, 1.464, 1.842, 2.085, 2.585, 2.050, 1.646, 1.540, 1.928, 2.548, 1.756, 1.958, 2.167, 1.536, 3.124, 1.670, 1.894, 1.354, 2.006, 2.719, 1.957, 1.670, 1.746, 1.548, 1.860, 1.988, 1.530, 2.001, 1.750, 2.798, 1.767, 1.806, 1.335, 1.775, 2.139, 1.885, 1.570, 1.735, 1.756, 1.702, 2.553, 2.066, 1.471, 2.093, 1.655, 2.856, 1.589, 1.439, 1.760, 1.887, 2.733, 2.140, 1.627, 1.794, 1.614, 1.881, 2.416, 1.908, 1.867, 1.727, 3.198, 1.584, 1.799, 1.356, 1.994, 2.743, 2.053, 1.648, 1.747, 2.422, 1.709, 2.052, 1.622, 1.950, 1.555, 2.999, 1.684, 1.712, 1.490, 1.767, 2.123, 2.107, 1.680, 1.572, 1.622, 1.848, 2.579, 2.007, 2.080, 1.558, 3.150, 1.660, 1.303, 1.889, 1.983, 2.697, 1.920, 1.758, 1.691, 1.745, 2.439, 1.882, 1.910, 1.751, 2.984, 1.667, 1.753, 1.361, 2.065, 2.757, 1.868, 1.569, 1.720, 1.661, 2.544, 1.831, 2.170, 1.428, 2.938, 1.658, 1.879, 1.469, 1.728, 1.879, 2.166, 1.552, 1.717, 1.616, 2.410, 2.038, 1.460, 1.895, 1.776, 3.090, 1.616, 1.369, 1.905, 1.956, 2.871, 1.986, 1.683, 1.674, 1.779, 1.774, 2.310, 1.685, 2.098, 1.925, 1.613, 1.737, 1.756, 1.424, 2.007, 2.635, 2.104, 1.718, 1.670, 1.548, 2.630, 1.751, 1.898, 1.481, 2.057, 1.590, 3.177, 1.924, 1.315, 1.877, 2.087, 1.984, 1.678, 1.749, 1.611, 1.792, 1.880, 1.641, 2.072, 1.658, 2.814, 1.700, 1.375, 1.683, 2.172, 2.794, 1.940, 1.596, 1.650, 1.732, 1.709, 1.890, 2.152, 2.043, 1.602, 2.930, 1.596, 1.831, 1.445, 1.955, 2.774, 2.019, 1.647, 1.724, 1.654, 2.391, 1.957, 1.945, 1.438, 2.009, 1.711, 1.529, 1.718, 1.916, 1.882, 1.974, 1.720, 1.648, 1.700, 2.306, 2.141, 1.535, 3.010, 1.778, 1.446, 2.060, 2.684, 2.140, 1.618, 1.610, 1.563, 1.886, 2.589, 1.712, 1.924, 2.094, 1.622, 3.102, 1.683, 1.830, 1.339, 2.639, 1.911, 1.696, 1.805, 1.609, 2.423, 1.629, 1.972, 1.788, 2.793, 1.715, 1.853, 1.301, 1.799, 2.066, 1.965, 1.607, 1.737, 1.699, 1.699, 2.661, 2.080, 1.433, 2.005, 1.628, 2.993, 1.545, 1.385, 1.777, 1.983, 2.110, 1.534, 1.740, 1.683, 1.941, 2.474, 1.859, 1.994, 1.973, 1.698, 3.063, 1.562, 1.750, 1.425, 1.939, 2.734, 1.736, 1.598, 1.745, 2.433, 1.747, 2.134, 1.639, 1.888, 1.566, 3.033, 1.762, 1.723, 1.405, 1.750, 2.060, 2.065, 1.619, 1.580, 1.944, 2.488, 1.910, 2.156, 1.605, 3.220, 1.635, 1.343, 1.929, 1.965, 2.554, 1.900, 1.736, 1.807, 1.544, 1.761, 2.450, 1.834, 2.068, 1.715, 2.902, 1.730, 1.828, 1.343, 2.063, 2.908, 2.016, 1.548, 1.676, 2.641, 1.783, 2.099, 1.435, 1.676, 2.837, 1.630, 1.847, 1.472, 1.775, 1.992, 2.006, 1.550, 1.798, 1.856, 2.277, 2.045, 1.466, 1.891, 1.721, 3.069, 1.586, 1.371, 1.914, 1.929, 2.799, 2.009, 1.763, 1.678, 1.709, 2.462, 1.810, 2.034, 1.882, 3.085, 1.688, 1.800, 1.432, 2.127, 2.607, 2.144, 1.611, 1.589, 1.634, 2.583, 1.706, 1.881, 1.527, 2.151, 1.569, 3.095, 1.619, 1.884, 1.371, 2.095, 1.918, 1.760, 1.715, 1.608, 1.680, 1.955, 1.637, 1.966, 1.685, 2.993, 1.726, 1.315, 1.698, 2.088, 2.876, 1.905, 1.658, 1.644, 1.719, 1.765, 2.489, 2.078, 2.165, 1.693, 2.917, 1.556, 1.863, 1.472, 1.878, 2.695, 2.077, 1.568, 1.794, 1.629, 2.322, 1.857, 1.454, 1.974, 1.652, 1.613, 1.764, 1.411, 1.842, 1.904, 2.041, 1.675, 1.593, 1.675, 1.847, 2.464, 2.126, 1.524, 1.885, 2.948, 1.765, 1.461, 1.871, 2.130, 2.619, 2.070, 1.600, 1.683, 1.587, 1.873, 2.564, 1.693, 1.924, 2.035, 1.616, 3.090, 1.933, 1.291, 1.930, 2.583, 1.971, 1.772, 1.793, 1.570, 2.529, 1.924, 1.926, 1.697, 2.962, 1.666, 1.851, 1.292, 1.773, 2.110, 1.969, 1.573, 1.711, 1.733, 1.754, 2.656, 2.057, 1.494, 2.138, 2.819, 1.527, 1.715, 1.986, 2.703, 2.119, 1.613, 1.721, 1.678, 1.831, 2.340, 1.948, 2.048, 1.919, 1.690, 3.183, 1.651, 1.691, 1.971, 2.891, 1.745, 1.597, 1.723, 2.304, 1.771, 2.064, 1.584, 1.941, 1.624, 1.682, 1.466, 1.855, 2.057, 2.067, 1.638, 1.659, 1.567, 1.881, 2.576, 1.950, 1.484, 2.154, 1.561, 3.171, 1.387, 1.828, 1.931, 2.677, 1.935, 1.694, 1.697, 1.585, 1.746, 2.494, 1.852, 1.980, 1.752, 2.875, 1.761, 2.174, 2.883, 1.907, 1.534, 1.756, 1.760, 2.490, 1.796, 2.084, 1.511, 2.017, 1.680, 2.843, 1.591, 1.932, 1.436, 1.772, 1.903, 2.151, 1.608, 1.778, 1.595, 1.830, 2.419, 1.980, 1.438, 1.936, 1.759, 3.172, 1.529, 1.958, 2.802, 2.058, 1.672, 1.606, 1.753, 1.842, 2.466, 1.707, 2.052, 1.983, 1.531, 2.984, 1.651, 1.730, 1.460, 2.175, 2.548, 2.072, 1.683, 1.592, 1.625, 2.582, 1.771, 1.987, 1.523, 2.053, 1.569, 3.191, 1.716, 1.828, 1.305, 1.856, 1.895, 1.738, 1.755, 1.554, 1.804, 2.443, 1.872, 1.615, 2.032, 2.951, 1.713, 1.363, 1.742, 2.009, 2.731, 1.897, 1.610, 1.753, 1.705, 1.791, 2.503, 1.809, 2.157, 2.147, 1.621, 2.909, 1.659, 1.448, 1.898, 2.108, 1.565, 1.741, 1.587, 2.470, 1.819, 2.076, 1.428, 1.947, 1.735, 3.059, 1.610, 1.689, 1.370, 1.934, 1.965, 1.704, 1.629, 1.763, 1.800, 2.354, 2.074, 1.649, 1.932, 1.580, 2.916, 1.725, 1.426, 2.077, 2.139, 1.658, 1.530, 1.836, 2.615, 1.767, 1.932, 2.015, 1.593, 3.177, 1.603, 1.926, 1.314, 2.062, 2.521, 1.963, 1.690, 1.759, 1.633, 2.533, 1.885, 1.896, 1.610, 2.056, 1.675, 2.898, 1.657, 1.794, 1.362, 1.678, 2.147, 1.624, 1.775, 1.724, 2.552, 2.091, 1.485, 2.035, 1.637, 3.007, 1.625, 1.395, 1.692, 1.934, 2.780, 2.096, 1.597, 1.745, 1.909, 2.335, 1.928, 1.923, 1.966, 1.781, 3.217, 1.532, 1.710, 1.439, 1.877, 2.720, 1.988, 1.635, 1.679, 2.273, 1.750, 2.166, 1.565, 1.977, 1.561, 3.018, 1.713, 1.817, 1.489, 1.778, 2.047, 2.146, 1.594, 1.592, 1.588, 1.845, 2.641, 1.976, 1.512, 2.067, 1.600, 3.073, 1.689, 1.337, 1.947, 2.088, 2.664, 1.880, 1.652, 1.785, 1.624, 1.736, 1.854, 1.961, 1.942, 1.777, 1.708, 1.813, 1.312, 2.062, 2.838, 1.990, 1.598, 1.723, 1.655, 2.663, 2.021, 1.446, 2.043, 1.651, 2.948, 1.573, 1.940, 1.407, 1.715, 1.967, 2.131, 1.573, 1.719, 1.929, 2.414, 1.478, 2.011, 1.677, 3.076, 1.586, 1.381, 1.839, 1.954, 2.819, 1.999, 1.778, 1.621, 1.723, 1.762, 2.381, 1.752, 2.139, 1.918, 1.556, 3.045, 1.746, 1.694, 1.421, 2.087, 2.662, 2.068, 1.705, 1.605, 2.533, 1.796, 1.859, 2.148, 1.625, 3.159, 1.635, 1.824, 1.374, 1.921, 1.989, 1.870, 1.688, 1.827, 1.536, 1.779, 2.401, 2.004, 1.521, 1.660, 2.898, 1.740, 2.879, 1.927, 1.563, 1.649, 1.708, 2.658, 1.778, 2.118, 2.137, 2.866, 1.877, 1.438, 1.949, 2.789, 2.036, 1.557, 1.771, 1.671, 1.842, 2.019, 1.498, 1.878, 1.772, 3.089, 1.593, 1.779, 1.343, 1.929, 1.887, 2.087, 1.740, 1.678, 1.684, 1.745, 2.393, 2.054, 1.561, 1.880, 1.617, 1.687, 1.431, 1.777, 2.159, 2.494, 2.163, 1.628, 1.588, 1.600, 1.911, 2.601, 1.709, 1.905, 2.139, 1.569, 3.069, 1.909, 1.366, 2.027, 2.605, 1.940, 1.723, 1.718, 1.645, 1.890, 1.966, 1.626, 1.988, 1.676, 2.980, 1.752, 1.307, 1.727, 2.104, 1.870, 1.610, 1.620, 1.743, 1.806, 2.528, 2.096, 1.459, 2.108, 1.674, 2.988, 1.562, 1.497, 1.778, 1.899, 2.619, 2.051, 1.561, 1.812, 1.624, 1.939, 2.351, 2.007, 1.941, 1.658, 3.116, 1.635, 1.788, 1.901, 2.881, 2.067, 1.698, 1.602, 1.684, 2.408, 1.695, 2.157, 1.531, 1.964, 1.613, 2.974, 1.758, 1.685, 1.434, 2.118, 2.023, 1.655, 1.655, 1.589, 1.832, 2.556, 1.552, 2.071, 1.632, 3.066, 1.620, 1.282, 1.928, 2.645, 2.002, 1.780, 1.803, 1.555, 1.715, 2.501, 1.938, 1.871, 1.988, 1.681, 2.940, 1.707, 1.845, 1.314, 2.139, 2.828, 1.953, 1.548, 1.718, 1.734, 2.589, 1.768, 2.038, 1.504, 2.123, 1.601, 2.807, 1.567, 1.878, 1.494, 1.713, 1.989, 2.098, 1.648, 1.742, 1.691, 1.848, 2.410, 2.042, 1.456, 1.899, 1.695, 3.206, 1.601, 1.852, 1.938, 2.894, 1.577, 1.723, 1.863, 2.343, 1.757, 2.047, 1.966, 1.618, 3.101, 1.708, 1.708, 1.468, 2.055, 2.596, 2.056, 1.665, 1.587, 2.538, 1.747, 1.980, 1.508, 2.134, 1.556, 3.144, 1.653, 1.920, 1.356, 1.834, 2.016, 1.698, 1.704, 1.531, 1.716, 2.513, 2.008, 1.565, 1.771, 2.787, 1.739, 1.807, 2.108, 2.904, 1.904, 1.526, 1.746, 1.682, 2.535, 1.759, 2.131, 2.046, 1.687, 2.881, 1.585, 1.906, 1.397, 1.907, 2.677, 2.144, 1.603, 1.780, 2.424, 1.943, 1.964, 1.425, 1.866, 3.200, 1.555, 1.776, 1.370, 1.889, 1.952, 2.072, 1.675, 1.643, 1.750, 2.450, 2.007, 1.608, 1.967, 1.566, 2.954, 1.461, 1.779, 2.105, 2.537, 2.066, 1.708, 1.617, 1.631, 1.858, 2.535, 1.792, 2.012, 2.046, 1.524, 1.701, 1.838, 1.295, 1.990, 2.664, 1.862, 1.761, 1.751, 1.582, 1.923, 1.877, 1.579, 2.056, 1.774, 2.940, 1.691, 1.766, 1.350, 2.082, 1.916, 1.595, 1.689, 1.647, 1.797, 2.507, 2.116, 1.439, 2.178, 1.608, 1.608, 1.501, 1.679, 1.925, 2.815, 2.105, 1.556, 1.739, 1.592, 1.892, 2.436, 1.862, 1.941, 1.731, 3.057, 1.621, 1.699, 1.396, 2.012, 2.866, 1.961, 1.695, 1.656, 1.781, 2.327, 1.703, 2.088, 1.603, 1.932, 1.608, 2.988, 1.816, 1.410, 1.801, 2.045, 2.090, 1.682, 1.660, 1.562, 1.881, 2.598, 1.862, 2.065, 1.575, 3.215, 1.641, 1.301, 1.850, 2.078, 2.005, 1.684, 1.781, 1.630, 1.768, 2.542, 1.875, 1.873, 1.693, 2.858, 1.684, 1.370, 2.736, 1.952, 1.637, 1.639, 1.722, 2.579, 1.836, 2.167, 1.506, 2.061, 2.957, 1.600, 1.849, 1.415, 1.723, 2.070, 1.605, 1.700, 1.675, 1.900, 2.377, 2.004, 1.487, 1.956, 1.736, 3.211, 1.526, 1.388, 1.958, 1.911, 2.735, 1.707, 1.632, 1.678, 1.856, 2.357, 1.756, 2.165, 1.943, 1.588, 1.759, 1.744, 1.487, 2.027, 2.160, 1.595, 1.628, 1.545, 2.645, 1.698, 1.976, 1.508, 2.068, 1.624, 3.072, 1.838, 1.888, 2.052, 1.917, 1.690, 1.806, 1.633, 1.734, 2.379, 1.921, 1.639, 1.957, 1.747, 2.886, 1.719, 1.298, 1.777, 2.008, 2.867, 1.981, 1.611, 1.737, 1.687, 1.681, 2.665, 1.824, 2.062, 2.085, 1.674, 2.948, 1.538, 1.935, 1.411, 1.977, 2.664, 2.157, 1.582, 1.745, 1.688, 2.408, 1.873, 1.983, 1.482, 1.977, 1.659, 3.056, 1.568, 1.728, 1.820, 1.986, 1.968, 1.724, 1.628, 1.741, 1.774, 2.380, 2.154, 1.614, 1.876, 1.536, 3.057, 1.743, 1.432, 2.668, 2.065, 1.672, 1.584, 1.594, 1.919, 2.517, 1.800, 1.871, 2.172, 1.628, 3.192, 1.593, 1.855, 1.385, 2.618, 1.862, 1.738, 1.764, 1.553, 2.405, 1.873, 1.927, 1.536, 2.072, 1.694, 2.952, 1.764, 1.837, 1.335, 1.698, 2.068, 1.541, 1.687, 1.705, 1.718, 2.598, 2.145, 1.439, 2.081, 1.700, 2.846, 1.614, 1.447, 1.757, 1.951, 1.590, 1.794, 1.678, 1.829, 2.281, 1.847, 2.022, 1.907, 1.770, 3.054, 1.583, 1.782, 1.373, 1.888, 1.759, 1.658, 1.681, 2.449, 1.782, 2.067, 1.558, 1.883, 1.572, 3.083, 1.672, 1.778, 1.399, 1.835, 2.155, 2.089, 1.623, 1.620, 1.952, 2.668, 1.921, 1.544, 2.119, 1.550, 3.089, 1.643, 1.376, 1.876, 2.021, 2.544, 1.724, 1.714, 1.620, 1.741, 2.509, 1.909, 1.969, 1.966, 1.662, 2.926, 1.752, 1.810, 1.288, 2.094, 2.836, 1.639, 1.727, 2.536, 1.818, 2.074, 1.455, 2.140, 1.667, 2.978, 1.564, 1.810, 1.477, 1.808, 1.878, 2.056, 1.824, 1.880, 2.354, 2.048, 1.424, 1.989, 1.695, 3.150, 1.618, 1.400, 1.824, 1.928, 2.876, 2.082, 1.563, 1.662, 2.420, 1.703, 2.109, 1.937, 1.624, 2.938, 1.760, 1.698, 1.441, 2.145, 2.679, 2.052, 1.599, 1.669, 1.630
